Convergence and Disruption in Digital Society -- Money, Secure Communication, Digital Objects and Generative AI in Spatial Mixed Reality

In the digital society's evolving landscape, open-source tooling and generative AI are pivotal in transforming global collaboration. These technologies promise to dismantle traditional barriers of accessibility, language, and governance, fostering an inclusive digital ecosystem. However, the journey towards a fully integrated digital society faces significant challenges, including trust, accessibility, and sustainable development. Emerging technologies like global ledgers and blockchain propose novel methods for transferring digital goods and personal data across diverse digital spaces. This development, coupled with augmented intelligence tools, aims to create decentralized and federated environments where creativity and collaboration can flourish. An "open metaverse" concept is gaining traction, promoting an alternative to restrictive proprietary platforms and emphasizing user empowerment and equity. Despite the opportunities, governance and ethical considerations remain paramount. The digital society must navigate the fine balance between innovation and the potential risks associated with new technologies. The drive for an inclusive, innovative, and secure digital society necessitates a commitment to open-source principles and ethical AI application. It also involves overcoming cultural, legislative, and technical barriers that impede global collaboration. The future digital society envisions a collaborative, inclusive, and innovative global community. By focusing on augmented intelligence and supported creativity, it aims to unlock new possibilities for economic empowerment, cultural exchange, and technological advancement. This vision is not without its challenges, but with continued commitment to ethical, open, and inclusive development, a more connected and empowered global community is within reach.

==> 03_adoption_table.tex <==
\begin{table}[]
\begin{tabular}{|l|r|l|r|}
\hline
\textbf{Country} & \textbf{\begin{tabular}[c]{@{}r@{}}\% of pop own\\ crypto\end{tabular}} & \textbf{Country} & \textbf{\begin{tabular}[c]{@{}r@{}}\% of pop own\\ crypto\end{tabular}} \\ \hline
Ukraine          & 12.7                                                                    & South Africa     & 7.1                                                                     \\ \hline
Russia           & 11.9                                                                    & Nigeria          & 6.3                                                                     \\ \hline
Venezuela        & 10.3                                                                    & Colombia         & 6.1                                                                     \\ \hline
Singapore        & 9.4                                                                     & Vietnam          & 6.1                                                                     \\ \hline
Kenya            & 8.5                                                                     & Thailand         & 5.2                                                                     \\ \hline
USA              & 8.3                                                                     & United Kingdom   & 5.0                                                                     \\ \hline
India            & 7.3                                                                     & Brazil           & 4.9                                                                     \\ \hline
\end{tabular}
\end{table}


==> 06_NIP.tex <==
\subsubsection{NIPS}
Much like Bitcoin it is the convention at this time to contribute through ``Nostr Implementation Possibilities'', or \href{https://github.com/nostr-protocol/nips}{`NIPs' via GitHub}. \par
User \href{https://stacker.news/k00b}{k00b} on \href{https://stacker.news/items/119948}{Stacker News} used GhatGPT to summarise the current proposals, and it's such a good list, and Nostr is so core to understanding this book and product, that it's worth duplicating here. It's entirely possible to skip this section, but it provides an excellent overview of the whole project at the time this snapshot was taken. This needs to be checked to see if it's right, work in progress. 

\begin{itemize}
\item NIP-01 - basic description: The Nostr Protocol is a protocol that defines the format and flow of communication between clients and relays. It includes a structure for events, which are the only object type in the protocol, and a set of messages that clients can send to relays over a WebSocket connection. Events have a specific format and are signed using Schnorr signatures with the secp256k1 curve. Clients can send three types of messages to relays: EVENT, REQ, and CLOSE. The EVENT message is used to publish events, the REQ message is used to request events and create subscriptions, and the CLOSE message is used to stop subscriptions. The REQ message includes a subscription id and a set of filters that determine which events are sent in the subscription. Relays are expected to store the filters and send all future matching events to the same WebSocket until it is closed or replaced by a new subscription.
\item NIP-02 - contact list event type: The Nostr Protocol defines a special event with kind 3, called the "contact list", which is a list of "p" tags representing profiles that a user is following. Each tag entry includes the public key of the profile, a relay URL where events from that key can be found, and a local name or "petname" for the profile. Contact lists can be used for a variety of purposes, including backing up a list of followed profiles, discovering and displaying lists of followed profiles, sharing relay information to increase censorship resistance, and constructing local "petname" tables for easier identification of profiles. When a new contact list is published, it overwrites any previous contact lists and should be stored by relays and clients.
\item NIP-03 - open timestamp attestations: The Nostr Protocol allows for the inclusion of OpenTimestamps (OTS) attestations in events. An OTS attestation is a timestamp that serves as evidence that a document existed at a specific point in time. To include an OTS attestation in an event, it can be added to the event body under the ots key as base64-encoded OTS file data. The event's ID should be used as the raw hash to be included in the OpenTimestamps merkle tree. OTS attestations can be provided by either clients or relays, and can be used to show that an event is at least as old as the OTS date.
\item NIP-04 - encrypted direct messages: The Nostr Protocol defines a special event with kind 4, called an "encrypted direct message", which is a message that is encrypted and intended for a specific recipient. The content attribute of the event should contain the base64-encoded, AES-256-CBC encrypted message, appended by the base64-encoded initialization vector as a querystring parameter. The tags attribute should contain an entry identifying the recipient of the message using the recipient's public key. The tags attribute may also contain an entry identifying the previous message in a conversation or a message that the encrypted message is explicitly replying to, using the event ID of the previous message. The message is encrypted using a shared cipher generated by combining the recipient's public key with the sender's private key.
\item NIP-05 - DNS based identifiers: The purpose of NIP-05 is to allow users to map their public keys to internet identifiers (email-like addresses) and vice versa. This allows clients to find a user's public key by searching for their internet identifier and display that identifier instead of the public key. The process involves making a GET request to a specific URL with the user's name as a query string. The response should include a JSON object with the names and public keys of users and optional relay URLs where the user can be found. Clients should primarily reference public keys rather than internet identifiers. This is an optional feature and is not mandatory for all clients to implement.
\item NIP-06 - mnemonic seed derivation: Outlines the process for generating a public key from a mnemonic seed phrase using the BIP39 and BIP32 standards. The BIP39 standard is used to generate a mnemonic seed phrase, which is then used to generate a binary seed. The BIP32 standard is then used to derive a specific path, m/44'/1237'/0'/0/0, from the binary seed. This process is the default method for generating a public key in a single-key client. However, other types of clients may use different derivation paths for different purposes.
\item NIP-07 - browser extension spec: is a proposal for an interface that can be used by web browsers and web-based applications to interact with Nostr-based systems. The interface includes methods for getting a user's public key, signing an event, and (optionally) getting a list of relay URLs and performing NIP-04 encrypted direct messaging. The interface is intended to be used by browser extensions such as nos2x and Alby, or by the Blockcore wallet.
\item NIP-08 - mentions: specifies a method for clients to handle mentions of other events and pubkeys in the content of text note events. When a client identifies a mention, it should add the pubkey or event ID to the tags array with the tag "p" and replace the textual reference in the content with the notation "[index]", where index is the 0-based index of the related tag in the tags array. When receiving a text note event with these mentions, the client can do a search-and-replace using the actual contents from the tags array and perform any desired context augmentation.
\item NIP-09 - deletion: describes an event kind for event deletion, which includes a list of event IDs for events to be deleted. The content field of the event may contain a text note explaining the reason for the deletion. Relays should delete or stop publishing any events with the same pubkey as the deletion request, and clients should hide or indicate a deletion status for the referenced events. Relays should continue to publish deletion events indefinitely and clients should broadcast deletion events to other relays that don't have them. Clients may choose to fully hide events referenced by valid deletion events or show the event with an indication that the author has "disowned" the event. A client must validate that the pubkey of each event referenced in the deletion request is identical to the pubkey of the deletion request before hiding or deleting the event. Relays may validate this as well, but are not required to do so. There is no "undelete" functionality.
\item NIP-10 - threaded replies: This NIP describes the proper use of "e" and "p" tags in text events, which helps clients display replies in a tree structure and track the pubkeys involved in a reply thread. The "e" tag may be positional or marked with "reply" or "root" to denote the event or root of a reply chain, and the "p" tag lists the pubkeys involved in a reply thread, including the pubkey of the event being replied to.
\item NIP-11 - relay self-description: Defines the format for a Relay Information Document, which is a JSON document provided by relays to clients to inform them of their capabilities, administrative contacts, and various server attributes. The document includes a name, a description, a public key for administrative contact, an alternate contact, a list of supported NIPs, information about the software used by the relay, and a version identifier. This document is provided to clients over HTTP when they make a request with the Accept header set to application/nostr plus json to a URI that supports WebSocket upgrades.
\item NIP-12 - arbitrary tag filters: suggests the addition of a feature to allow relays (server nodes in the Nostr network) to support subscriptions to arbitrary tags in events. This feature would allow clients to search for events based on specific tags, such as location or topic. The NIP specifies that only single-letter tags can be used in queries to avoid bloating the relay indexes and to allow for easier detection of any potential abuse of the feature. The NIP provides suggestions for possible uses of this feature, including a decentralized commenting system, location-specific posts, and hashtags. However, the NIP does not standardize the use of any specific tag for any particular purpose.
\item NIP-13 - PoW: proposes the use of Proof of Work (PoW) in Nostr notes as a means of deterring spam. PoW is a computation-based proof that can be universally validated by relays and clients, and it is added to notes to provide evidence of computational work. To generate PoW for a Nostr note, a nonce tag is added to the note, and the number of leading zero bits in the note's ID is used to determine the difficulty of the PoW. Clients can use the difficulty of a note's PoW to determine whether to accept or reject it, with higher difficulty indicating a higher level of computational work. Reference code for calculating the difficulty of a note's PoW is provided in the NIP. The NIP also suggests using prefix searches to filter notes by their PoW difficulty when querying relays.
\item NIP-14 - Subject tags: proposes the use of a "subject" tag in text events, which can be used in threaded lists of messages in browsers instead of using the first few words of the message. It is similar to how email clients display lists of incoming emails by subject. When replying to a message, the subject tag should be replicated, and clients may add text to denote that it is a reply. The subject should generally be shorter than 80 characters in length.
\item NIP-15 - End of stored events: proposes a method for relays to notify clients when all stored events have been sent. The relay will send the client a "EOSE" message after it has sent all the events it has persisted, indicating that all events coming after this message are newly published. Clients should use the "supported nips" field to determine if a relay supports this feature, which is intended to reduce uncertainty and potentially simplify client code by knowing when all events have been sent.
\item NIP-16 - regular/replaceable/ephemeral event types: proposes the creation of three categories of events: regular events, replaceable events, and ephemeral events. Regular events have a kind between 1000 and 10000, and upon being received by a relay, they are sent to all clients with a matching filter and are stored. Replaceable events have a kind between 10000 and 20000, and upon being received by a relay, if they have a newer timestamp and are signed by the same key as the currently known latest replaceable event with the same kind, the old event is discarded and replaced with the newer event. Ephemeral events have a kind between 20000 and 30000, and upon being received by a relay, they are sent to all clients with a matching filter but are not stored. Clients should use the "supported nips" field to determine if a relay supports these event categories, and should not send ephemeral events to relays that do not support this NIP as they may be persisted. Replaceable events may be sent to relays that do not support this NIP, and clients querying should be prepared to receive multiple events and use the latest one. These event categories may be used in various applications such as states, typing indicators, and messaging.
\item NIP-18 - reposts: proposes the use of "reposts," which are kind 6 notes that signal to followers that another event is worth reading. The content of a repost event is empty, and it must include an "e" tag with the ID of the note being reposted, as well as a "p" tag with the pubkey of the event being reposted. The "e" tag should also include a relay URL as its third entry to indicate where it can be fetched.
\item NIP-19 - bech32/human readable encoding of keys/ids/etc: proposes the use of bech32-formatted strings to display keys, IDs, and other information in clients. These formats are not intended to be used in the core protocol, but rather for displaying to users, copy-pasting, sharing, rendering QR codes, and inputting data. It is recommended that IDs and keys be stored in hex or binary format for use in the core protocol. The NIP defines three bech32 prefixes for bare keys and IDs: "npub" for public keys, "nsec" for private keys, and "note" for note IDs. The NIP also defines two bech32 prefixes with TLV (type-length-value) contents for shareable identifiers with extra metadata: "nprofile" for nostr profiles and "nevent" for nostr events. Standardized TLV types are defined for these prefixes, including "special" for the key or ID of the profile or event, and "relay" for a relay where the entity is more likely to be found. These bech32 encodings are not intended to be used inside the standard NIP-01 event formats or filters, but are meant for human-friendly display and input. Clients should accept keys in both hex and npub format for now and convert them internally.
\item NIP-20 - event responses: proposes the introduction of "command results," which provide more information about whether an event was accepted or rejected by a relay when it is submitted. A command result is a JSON object with the structure ["OK", event id, true/false, message], where "OK" indicates that the event was either successfully saved to the database or rejected, event id is the ID of the event, true/false indicates whether the event was a duplicate and has already been saved, and message provides additional information about the success or failure of the command. Possible values for message include "duplicate," "blocked," "invalid," "pow," "rate-limited," and "error." Clients should handle these messages differently based on the prefix, such as showing error popups for "invalid" or "blocked," querying relay metadata for updated difficulty requirements for "pow," or trying again with a longer timeout for "rate-limited." Ephemeral events are not acknowledged with "OK" responses unless there is a failure. If the event or "EVENT" command is malformed and cannot be parsed, a NOTICE message should be used instead of a command result. This NIP only applies to non-malformed "EVENT" commands.
\item NIP-22 - timestamp limits: proposes a standard for relays to set limits on the timestamps of events they are willing to store. The limits would be specified as unix timestamps in seconds and would apply to all events, including regular and replaceable events. If a relay supports this NIP, it would send a command result to the client indicating whether an event was accepted or rejected due to its created at timestamp falling outside the permitted range. Clients can use the supported nips field to determine whether a relay uses event created at time limits and can handle command results accordingly. The motivation for this NIP is to improve the user experience by decreasing the number of events that appear out of order or from impossible dates in the past or future.
\item NIP-25 - reactions: A reaction is a type of note used to express a positive or negative sentiment towards another note. The content of a reaction event can be a "+" or "-", which indicates a "like" or "dislike" respectively, or an emoji. The reaction event should include the "e" and "p" tags from the note being reacted to, allowing users to be notified of reactions to their posts and enabling clients to retrieve all reactions for a specific post or thread. The "e" tag should include the ID of the note being reacted to, and the "p" tag should include the pubkey of the event being reacted to.
\item NIP-26 - delegation: describes a way for events to be signed by keypairs other than the ones that are normally used. This can be used to allow a user to generate new keypairs for each client they use, and authorize those keypairs to generate events on behalf of their root pubkey (a keypair that is stored in a secure location). The proposal introduces a new "delegation" tag that can be included in events to indicate that the event has been signed by a delegate keypair on behalf of another keypair. The proposal also describes the process for creating and using a "delegation token", which is a signature that grants authorization for the delegate keypair to sign events on behalf of the delegator.
\item NIP-28 - chat: defines new event kinds for public chat channels, messages in those channels, and basic moderation of those channels. The proposal reserves five event kinds for immediate use and five event kinds for future use. These event kinds include: creating a chat channel, setting metadata for a chat channel, sending a message in a chat channel, hiding a message in a chat channel, and muting a user in a chat channel. The proposal outlines how each of these event kinds should be used, including the data that should be included in the event and how clients and relays should handle the events.
\item NIP-33 - further replaceable events standards: adds a new range of event kinds that allow for the replacement of events that have the same "d" tag and kind. This is an extension of NIP-16, which only allowed for the replacement of events with the same kind. The proposal defines a "parameterized replaceable event" as an event with a kind of 30000 or greater, but less than 40000. The proposal outlines how these events should be handled by clients and relays, including the use of the "supported nips" field to determine support for this NIP and the use of tag filters to handle multiple events.
\item NIP-36 - Content warning: introduces the "content-warning" tag, which allows users to specify that the content of an event requires approval by readers before it is shown. The proposal describes how the tag should be used, including the optional inclusion of a "reason" for the content warning. This tag can be used by clients to hide the content of the event until the user has approved it.
\item NIP-40 - expiring events: introduces the "expiration" tag, which allows users to specify a unix timestamp at which an event should be considered expired and deleted by relays. The proposal outlines how the tag should be used, including the format of the timestamp and how it should be interpreted. The proposal also describes the behavior that clients and relays should follow when working with expired events, including the use of the "supported nips" field to determine support for this NIP and the requirement for relays to drop expired events that are published to them. The proposal suggests potential use cases for the expiration tag, including temporary announcements and limited-time offers. The proposal notes that expired events may still be accessible to third parties through the relays, and warns against using the expiration tag as a security feature.
\end{itemize}


==> 07_1_NFTUmran.tex <==
\textbf{NFT Use Cases}

\textbf{Art}

The recent surge of interest in NFT's during early 2021 has largely been
driven by digital art NFT's, despite the origins of digital art NFT's
started much earlier in 2014. New York artist
\href{https://www.mccoyspace.com/project/125/}{Kevin McCoy's
\emph{Quantum}} is widely recognised as the first piece of art created
as an NFT. However it was during early 2021 that art NFT's started to
gain significant attention; by the end of 2021, nearly
\href{https://www.paymentscardsandmobile.com/state-of-the-blockchain-nfts-explode-onto-scene-in-2021/}{£31b
had been spent} on NFT purchases, a considerable and exponential growth
given
\href{https://raritysniper.com/news/nfts-exploded-in-2021-with-25-billion-in-sales/}{2020
sales of \textasciitilde£71m}

High profile digital artists such as \emph{Beeple} whose
\href{https://www.forbes.com/sites/abrambrown/2021/03/11/beeple-art-sells-for-693-million-becoming-most-expensive-nft-ever/?sh=3f237d1c2448}{recent
recording break sale} of his NFT \emph{``The first 5000 days''} (Figure \ref{fig:first5000days}) at Christies (a long established British auction house,
specialising in high profile precious work of art) for £52.9m helped
bring NFT's into the public spotlight and wider give them global
attention.

\begin{figure*}[ht]\centering % Using \begin{figure*} makes the figure take up the entire width of the page
	\includegraphics[width=\linewidth]{first5000days}
	\caption{Beeple: First 5000 days, \href{https://onlineonly.christies.com/s/beeple-first-5000-days/lots/2020}{taken from the Christies website, assumed fair use}.}
	\label{fig:first5000days}
\end{figure*}

Art as NFT's offer the following advantages:

\begin{enumerate}
\def\labelenumi{\arabic{enumi}.}
\item
  \textbf{Immutable Nominal Authenticity:} Art fraud such as false
  representation, forgeries, plagiarism have been a reoccurring blight
  since art has existed; artists and works of art have been open to
  abuse by forgers, black market profiteers and even fellow artists
  laying claim to works of art of others. Unless a work of art is sold,
  exhibited or listed, documenting when and who created it, the
  \emph{nominal authenticity,} which Dutton states as the
  \emph{``correct identification of the origins, authorship, or
  provenance of an object''} \cite{dutton2003authenticity} can be increasingly mutable over a period
  of time, dependent on a multitude of factors, including; the artists
  existing profile, how widely and where the work of art is exhibited,
  if the work of art is commissioned by a patron, if it's sold, and
  profile of the buyer/collector. At its most basic level, once a work
  of art is `minted' as an NFT (publishing the art work as a unique
  token on the blockchain) this functions as an immutable publicly
  accessible proof of ownership and by extension proof of creation. The
  act of minting is not purely limited to digital art; all an artist
  requires is a digital representation of any physical art (sculpture,
  physical painting, installation etc..) which can be used as a proxy
  allowing artists to record the date of creation/origin of a physical
  piece of art on the blockchain, a buyer purchasing the NFT can be
  provided the actual physical artwork as part of the NFT. Nominal
  authenticity becomes secure and immutable.

  \begin{enumerate}
  \def\labelenumii{\alph{enumii}.}
  \item
    \textbf{Secure Digital Provenance}:
    \href{https://en.wikipedia.org/wiki/Provenance}{Provenance} (or the
    chain of custody) is an important aspect in works of art, antiques
    and antiquities. Provenance not only helps assign work to an artist
    but also documents ownership history. Digital provenance, an
    inherent feature of NFT's means provenance now no longer becomes
    what has historically sometime been a contentious detective's game
    at the best of times; one that is open to fraud, misinterpretation
    and entirely reliant on good record keeping.
  \end{enumerate}
\end{enumerate}

\begin{quote}
Since provenance can contribute to the value of a piece of art
(benefiting both the creator and collector) the use of the blockchain as
an open, secure ledger is a far more trustworthy system than traditional
methods of artistic provenance that were cobbled together; often
consisting of a mix of physical and digital documents spanning private
\& public sale receipts, art/museum gallery exhibitions and private
record keeping). Digital provenance provided when an artist `mints' a
piece of art into an NFT allows artists and collectors to record a
secure, permanent unalterable history of transactions for a specific
piece of art, providing future collector complete trust in the origin
and custody of a piece of art.
\end{quote}

\begin{enumerate}
\def\labelenumi{\alph{enumi}.}
\setcounter{enumi}{1}
\item
  \textbf{Decentralised automated royalty payments}: Traditionally if a
  piece of art is sold, the first sale may (but not always) benefit the
  artist financially, however secondary and any subsequent sales would
  only ever financially benefit the buyer/collector; the original artist
  would rarely benefit. However If a work of art is minted into an NFT,
  royalty payments can be predetermined and automated in perpetuity
  directly by the use of a `smart contract'. Smart contracts are small,
  automated scripts/programs that run automatically and independently of
  a buyer/seller; pre-determined conditions are set by the buyer; these
  trigger when certain conditions are met i.e

  \begin{enumerate}
  \def\labelenumii{\roman{enumii}.}
  \item
    \emph{On sale transfer 20\% of total sale amount into digital wallet
    of the creator.}
  \item
    \emph{On sale transfer 80\% of total sale amount into digital wallet
    of the seller.}
  \end{enumerate}
\end{enumerate}

\begin{quote}
Once the royalty payment rate is set by the artist/creator, future
royalties of all sales can be paid directly to the artist/creator
account (via a digital wallet) without the need of a third party
(traditionally a gallery/agent etc..).

Smart contract driven NFT's means that even if piece of art is resold 5,
10 or even a 100,000 times moving through 5, 10 or even a 100,000
different collectors; a pre-determined royalty payment rate set by the
creator would still guarantee the artist/creator is paid directly from
each and every future sale.

Historically provenance for works of art may span across generations,
for instance Gabriël Metsu's oil on canvas painting \emph{The Lace
Maker's} provenance, first recorded in 1722, now spans 300 years of
ownership, including from a British Baron in the 19\textsuperscript{th}
century to an American philanthropist in the 20\textsuperscript{th}
century.) Metsu died young at the age of 38, leaving a widow; neither
his/her relatives/descendants benefit from his original work, 300 years
later this would be near impossible to facilitate with traditional
systems, as even legal contracts are open and prone to the ravages of
time.

NFT smart contracts hold an incredibly potential; an artists descendants
financially benefiting directly from the resale of a piece of work long
after the artist/museum's/gallery or even state have turned to dust as
long as the original creator's digital wallet is accessible, \emph{the
blockhain becomes an everlasting digital patron} ensuring
\end{quote}

\textbf{Computer \& Video Games}

Computer \& Video games are a huge global business, exponential global
growth over the last 30 years has seen this grow to a point where it has
eclipsed both the
\href{https://www.businessinsider.com/video-game-industry-revenues-exceed-sports-and-film-combined-idc-2020-12?r=US\&IR=T}{global
movie and North American sports industries} combined.

A global industry with revenues over £120b,
\href{https://www.wepc.com/news/video-game-statistics/}{with
\textasciitilde half the people on the planet} playing some form of
games in 2021.

As the games industry has evolved and matured over the last 40 years,
secondary markets have emerged, most notably the `second hand' games
resale market. The rise of `retro' gaming, has demonstrated the second
hand market is a lucrative one for private resellers, an unopened copy
of Super Mario Bros for the Nintendo Entertainment System
\href{https://www.nytimes.com/2021/08/06/business/super-mario-bros-sale-record.html}{recently
selling for £1.5M} to the extent the market has seen
\href{https://www.businessinsider.com/retro-gaming-market-being-overtaken-by-speculators-2021-9?r=US\&IR=T}{speculators
looking to cash in} on the huge global interest in retro/second hand
games

Despite publishers and developers increasingly moving to non-physical
digital only' games, the demand for used games remains incredibly high.

Whilst some retailers have adapted their business models to include
reselling of retro/second hand games, the vast majority of
publisher/developers/retailers aren't able to directly benefit from the
emerging retro/second hand games market. The potential of \emph{video
games as NFT's} presents a huge opportunity for publishers, developers
and players alike, offering the following advantages:

\begin{enumerate}
\def\labelenumi{\alph{enumi}.}
\item
  \textbf{Royalty Sales on Pre-owned Games} ; A predetermined proportion
  of any resale of a used game can automated in perpetuity via smart
  contracts; once these are set by the publisher, future royalties of
  all sales can be paid directly to the publishers/developers wallets (a
  digital account) without the need of a third party (traditionally a
  retail entity). Traditionally only the initial first sale of a game
  would financially benefit the publisher/developer/retailer, secondary
  and subsequent sales would only ever financially benefit the
  purchaser, with many developers/publishers arguing this is hurting the
  wider industry through the loss of significant income generated by the
  secondary and subsequent sales, sometimes over the course of decades.
  However the use of NFT's smart contracts means that if a game is
  sold/resold through 10,000 collectors; a pre-determined royalty
  payment rate set by the publisher would still guarantee the publisher
  (and or developer/retailer) takes a proportion of any future sales.
\item
  \textbf{Monetisation of User Generated Content:} Games as a NFT's
  offer ability to monetise UGC: User generated content.
\end{enumerate}

\begin{quote}
Video games such as
\href{https://www.businessofapps.com/data/pokemon-go-statistics/}{Nintendo's
\emph{Pokemon Go}} \emph{(166 million players)},
\href{https://techacake.com/destiny-2-player-count/\#:~:text=The\%20total\%20player\%20base\%20of,to\%20be\%2038\%20million\%20players.\&text=According\%20to\%20the\%20source\%2C\%20the,in\%20terms\%20of\%20player\%20population.}{Bungie's
\emph{Destiny 2}} \emph{(38 million players)} or
\href{https://fictionhorizon.com/how-many-people-play-genshin-impact/\#:~:text=Genshin\%20Impact\%20had\%20approximately\%209,million\%20users\%20in\%20June\%202021.}{miHoYo's
Genshin Impact} (\emph{9 million players} ) all have large, established
and significant player bases. What is noteworthy, the games are designed
to encourage players may spend hundreds, or in some cases thousands of
hours on one game alone; according to
\href{https://destinytracker.com/destiny/leaderboards/all/minutesplayedtotal?grouped=true\&page=1}{Destinytracker.com},
the top players have amassed total play times over 20,000 hours, close
to 1,000 days or \textasciitilde{} 3 years, which is incredible feat
given Destiny 2 only launched 5 years ago in 2017.

Destiny/Pokemon Go and Genshin Impact revolve around a central key game
mechanic; players investing significant amounts of time collecting in
game digital assets; characters/weapons/items, often classed as `rare'
or `exotic' or `5 Star'. These collectibles usually found by a
combination of the accrual of in-game time, completing quests,
purchasing additional in-game items/boosters, and luck (`RNG'). Players
are often encouraged to share their collections of rare
characters/weapons/ objects through in-game achievements, triumphs,
scores acting as a mark of distinction/status symbol.

Traditionally there has been nothing that went beyond sharing the
\emph{digital badge} (i.e triumph/achievement/accomplishment) on a on
social media/gamer's platform profile. However NFT's offer the ideal
system for developers/publishers and even players to monetise user
generated/customised data (such as a players unique save game data),
simultaneously allowing:

a) creation of an additional monetised ecosystem to meet player demands
i.e. some players who are willing to monetise and `sell' their invested
time in a particular product/service to other players with little time
but willing to pay other players for `grinding' (progressing laborious
in game tasks) and a more advanced in-game progression point.

The potential to provide publishers/developers with an additional
long-term income stream, providing a better ROI on computer \& video
game development, which in many instances can cost hundreds of millions
in development costs spanning 5/10 years, is undeniable.
\end{quote}

\begin{enumerate}
\def\labelenumi{\alph{enumi}.}
\setcounter{enumi}{2}
\item
  Play to earn revenue models.
\item
  Monetizing In game collectibles: customisable in game assets (vanity
  items such as cosmetic character skins/clothing or collectible items
  that offer player advantages(new weapons/vehicles/mods etc,..)
\end{enumerate}

\textbf{Figure 1.x:} Typical Smart Contract Structure:
https://www.jigsawllc.com/2021/03/25/nfts-creativity-innovation/


==> 08_metaverse_extra.tex <==

\section{History and market need}

The word metaverse was coined by the author Neal Stephenson in his 1992 novel Snowcrash. It started popping up soon after in \href{https://www.newscientist.com/article/mg14819994-000-how-to-build-a-metaverse/}{news articles} and research papers \cite{mclellan1993avatars}, but in the last five years it has been finding a new life within a silicon valley narrative.\par
There were clear precursors to modern social VR, such as \href{https://www.howtogeek.com/778554/remembering-vrml-the-metaverse-of-1995/}{VRML in the 1990's} which laid much of the groundwork for 3D content over networked computers.\par% The author used to create commercial 3D scenes on Silicon Graphics systems back in the late 90s.\par
It might seem that there would be a clear path from there to now, in terms of a metaverse increasingly meaning connected social virtual spaces, but this has not happened. Instead interest in metaverse as a concept waned, MMORG (described later) filled in the utility, and then recently an entirely new definition emerged. The concept of the Metaverse is extremely plastic at this time (Figure \ref{fig:muskWeb3}). This book will aim to build toward an understanding of metaverse which really means a useful social mixed reality layer, that allows low friction communication and economic activity, within groups, at a global scale. This focus on value and trust means it's most appropriate to focus on business uses.\par
This chapter will attempt to frame the context for telepresence (the academic term for communicating through technology), and then explain the increasingly polarised options for metaverse. It's useful to precisely identify the primitives of the product we would like to see here, so this chapter is far more a review of academic literature in the field, culminating in a proposed framework.\par
\begin{figure}
  \centering
    \includegraphics[width=\linewidth]{muskWeb3}
  \caption{Elon Musk agrees with this on Twitter. It's notable that Musk is now Twitters' \href{https://twitter.com/paraga/status/1511320953598357505}{biggest shareholder}, and has been vocal about web censorship on the platform.}
  \label{fig:muskWeb3}
\end{figure}
\input{08_b2b_telepresence}    
\section{Post `Meta' metaverse}
The current media around ``metaverse'' has been seeded by Mark Zuckerberg's rebranding of his Facebook company to `Meta', and his planned investment in the technology. The second order hype is likely a \href{https://www.goldmansachs.com/insights/pages/framing-the-future-of-web-3.0-metaverse-edition.html}{speculative play} by major companies on the future of the internet. Some notable exerts from a \href{https://www.jpmorgan.com/content/dam/jpm/treasury-services/documents/opportunities-in-the-metaverse.pdf}{2021 report} by American bank JPMorgan show how the legacy financial institutions see this opportunity:\par
\begin{itemize}
\item In the view of the report \textit{``The metaverse is a seamless convergence of our physical and digital lives, creating a unified, virtual community where we can work, play, relax, transact, and socialize.'' - this isn't the worst definition, and very much plays into both the value and mixed reality themes explored in this book.}
\item They agree with the industry that monetisation of assets in metaverse applications is called ``Metanomics''. It's worth seeing this word once, as it's clearly gaining traction, but it won't be used in this book.
\item They make a point which is at the core of this book, that value transaction within metaverses may remove effective border controls for working globally. Be this teleoperation of robots, or shop fronts in a completely immersive VR world. They say: \textit{``One of the great possibilities of the metaverse is that it will massively expand access to the marketplace for consumers from emerging and frontier economies. The internet has already unlocked access to goods and services that were previously out of reach. Now, workers in low-income countries, for example, may be able to get jobs in western companies without having to emigrate.''}
\item There is a passage which foreshadows some of the choices made in this book: \textit{``Expanded data analytics and reporting for virtual spaces. These will be specifically designated for commercial and marketing usage and will track business key performance indicators (this
already exists in some worlds, such as Cryptovoxels)''}. More on this later.
\item The report attempts to explore the web3 \& cryptocurrency angles of metaverse. That's also the aim of this book, but they have taken a much more constrained approach, ignoring the possibilities within Bitcoin.
\item They assert that strong regulatory capture, identification, KYC/AML etc should underpin their vision of the metaverse. This is far from the community driven and organically emergent narratives that underpin Web3. This is their corporate viewpoint, something they have to say. On the back of this they pitch their consultancy services in these areas.
\end{itemize}

There has been a reactive pushback against commercialisation and corporateisation by the wider tech community, who are concerned about the aforementioned monetisation of biometrics. \href{https://www.coindesk.com/layer2/2022/01/19/meta-leans-in-to-tracking-your-emotions-in-the-metaverse/}{Observers do not trust} these `web' players with such a potentially powerful social medium. It is very plausible that this is all just a marketing play that goes nowhere and fizzles out. It is by no means clear that people want to spend time socialising globally in virtual and mixed reality. These major companies are  making an asymmetric bet that if there is a move into virtual worlds, then they need to be stakeholders in the gatekeeping capabilities of those worlds.\par 
Meta,Disney plus, Sportswear manufacturers\par

\href{https://medium.com/kabuni/fiction-vs-non-fiction-98aa0098f3b0}{Can enough be done to prevent abuse?}

It seems like there are four major interpretations of the word.\par

Facebook have recently rebranding their parent company as `Meta' and they are aggressively promoting ``The Metaverse'' as a shared social VR space, chiefly of their design. In Stephenson's `Snow Crash' the Hero Protagonist (drolly called Hiro Protagonist) spends much of the novel in a dystopian virtual environment called the metaverse. It is unclear if Facebook is deliberately embracing the irony of aping such a dystopian image, but certainly their known predisposition for corporate surveillance, alongside their attempt at a global digital money is ringing alarm bells.\par
The Grayscale investment trust \href{https://grayscale.com/wp-content/uploads/2021/11/Grayscale_Metaverse_Report_Nov2021.pdf}{published a report} which views Metaverse as a potential trillion dollar global industry. Such industry reports are given to hyperbole, but it seems the technology is becoming the focus of technology investment narratives.
\subsection{Mixed reality as a metaverse}
\href{https://docs.microsoft.com/en-us/windows/mixed-reality/design/spatial-anchors}{Spatial anchors} allow digital objects to be overlaid persistently in the real world. With a global `shared truth' of such objects a different kind of metaverse can arise.
One such example is the forthcoming \href{https://avvyland.com/}{AVVYLAND}.

Peleton as a metaverse?


\section{Immersive and third person XR}
In considering the needs of business to business and business to client social VR is it useful to compare software platforms:
\subsubsection{Second Life}
Notable because it's the original and has a decently mature marketplace. Some \$80B was \href{https://www.zdnet.com/article/high-fidelity-invests-in-second-life-to-expand-virtual-world/}{paid to creators} in Second Life in 2021 in a wider economic ecosystem of around \$650M.
\subsubsection{Roblox}
Around 60 billion messages are \href{https://podcasts.apple.com/us/podcast/developments-investments-experiences-in-the-metaverse/id1593908027?i=1000540906629}{sent daily} in Roblox 

\subsubsection{Spatial}
\begin{itemize}
\item Very compelling. Wins at wow.
\item Great avatars, user generated
\item AR first design
\item Limited scenes
\item Smaller groups (12?)
\item Limited headset support
\item Intuitive meeting support tools
\item No back end integration
\end{itemize}
\subsubsection{MeetinVR}
\begin{itemize}
\item Good enough graphics, pretty mature system
\item OK indicative avatars, user selected
\item VR first design
\item Limited scenes
\item Smaller groups (12?)
\item Quest and PC
\item Writing and gestures supported
\item Some basic enterprise tools integration
\item Bring in 3D objects
\item Need to apply for a license?
\end{itemize}
\subsubsection{Glue}
\begin{itemize}
\item Better enterprise security integration
\item Larger environments, potential for breakouts in the same space. Workshop capable
\item 3D object support, screen sharing, some collaborative tools
\item Apply for a license
\item Fairly basic graphics
\item Basic avatars
\item Quest and PC
\item Writing and gestures supported
\item Mac support
\end{itemize}
\subsubsection{Mozilla Hubs}
\begin{itemize}
\item Open source, bigger scale, more complex
\item Choose avatars, or import your own
\item Environments are provided, or can be designed
\item Useful for larger conferences with hundreds or thousands of members but is commensurately more complex
\item Quest and PC
\item Larger scenes within scenes
\end{itemize}
\subsubsection{FramesVR}
\begin{itemize}
\item Really simple to join
\item Basic avatars
\item Bit buggy
\item 3D object support, screen sharing, some collaborative tools
\item Quest and PC
\item Larger scenes within scenes
\item Runs in the browser
\end{itemize}
\subsubsection{AltSpace}
\begin{itemize}
\item Microsoft social meeting platform
\item Very good custom avatar design
\item Great world building editor in the engine
\item Doesn't really support business integration so it's a bit out of scope
\item Huge numbers (many thousands) possible so it's great for global events
\item Mac support
\end{itemize}
\subsubsection{Engage}
\begin{itemize}
\item Great polished graphics
\item Fully customisable avatars
\item Limited scenes
\item Presentation to groups for education and learning
\item PC first, quest is side loadable but that's a technical issue
\item BigScreen VR
\item Seated in observation points in a defined shared theatre
\item Screen sharing virtual communal screen watching, aimed at gamers, film watching
\item up to 12 user
\end{itemize}
\subsubsection{VRChat}

\subsubsection{NEOSVR}
\href{https://neos.com/}{Notable because} it's trying to integrate crypto marketplaces
\subsubsection{Meta Horizon Worlds \& Workrooms}
Horizon Worlds is the Meta (Facebook) meteverse, and Workrooms it's business offering and a subset of the ``Worlds'' global system. It is currently a walled garden without connection to the outside digital world, and arguably not therefore a metaverse.\par
The Financial Times \href{}{took a look} at their patent applications and noted that the travel is toward increased user behaviour tracking, and targeted advertising.\par
Facebook actually have a poor history on innovation and diversification of their business model. This model has previously been tracking users to target ads on their platform, while increasing and maintaining attention using machine learning algorithms. \par
It makes complete sense then to analyse the move by Meta into 3D social spaces as an attempt to front run the technology using their huge investment capacity. Facebook have recently taken a huge hit to their share price. Nothing seems to changed in the underling business except Zuckerbergs well publicised shift to supporting a money losing gamble on the Metaverse. It is by no means clear that users want this, that Meta will be able to better target ads on this new platform, or that the markets are willing to trust Zuckerburg on this proactive move. \par
With all this said the investment and management capacity and capability at Meta cannot be dismissed. It is very likely that Meta will be able to rapidly deploy a 3D social space, and that it's development will continue to be strong for years. The main interface for Horizon Worlds is through the Meta owned and developer Oculus headset, which is excellent and reasonably affordable. It has been quite poorly received \href{https://kotaku.com/facebook-metaverse-horizon-worlds-vr-oculus-quest-2-cha-1848436740}{by reviewers} but will likely improve, especially if users are encouraged to innovate.
\subsubsection{Webaverse}
\href{https://webaverse.com/}{Webaverse} are an open collective using open source tools to create interoperable metaverses.
\subsubsection{Vircadia}
We have chosen Vircadia as our development platform for this investigation is it's a community supported free and open source project with some support for economic interaction.


\section{Digital Land Metaverses}
One of the most intuitive ways to view a metaverse is as a virtual landscape. This is how metaverse was portrayed in the original Neal Stephenson use of the word. 
\section{Global enterprise perspective}
Microsoft have just bought Activision / Blizzard for around seventy billion dollars. This has been communicated by Microsoft executives as a ''Metaverse play'', leveraging their internal game item markets, and their massive multiplayer game worlds to build toward a closed metaverse experience like the one Meta is planning.
This builds on the success of early experiments like the Fornite based music concerts, which attracted millions of concurrent users to live events.

\section{NFT as metaverse narrative}
Within the NFT community it is normalised to refer to ownership of digital tokens as participation in a metaverse. 
This CNBC article highlights the confusion, as this major news outlet refers to \href{https://www.cnbc.com/2022/01/16/walmart-is-quietly-preparing-to-enter-the-metaverse.html}{Walmart prepares to offer NFTs}'' as an entry ``into the metaverse''.

\section{MMORG games and NFTs}
Traditional gamers have pushed back on the seemingly useful idea of integrating NTFs with traditional games. This may be in part because Ethereum mining has kept graphics card prices high for a decade.

\href{https://www.prnewswire.com/news-releases/hbar-foundation-and-ubisoft-partner-to-support-growth-of-gaming-on-hedera-network-301474971.html}{HBAR partnerships}
The \href{https://twitter.com/justinkan/status/1491270239967154178}{following text} is from Justin Kan, co-founder of twitch: \textit{``NFTs are a better business model for games. Many gamers seem to be raging hard against game studios selling NFTs. But NFTs are also better for players. Here’s why I think blockchain games will be the predominant business model in gaming in ten years. NFTs are a better business model for funding games . Example: recently I invested in a new web3 game SynCityHQ. They are building a mafia metaverse and raised \$3M in their initial NFT drop.\\ NFTs give studios access to a new capital market for raising capital from the crowd.NFTs can be a better ongoing model for games. Web3 games will open economies, and by building the games on open and programmable assets (tokens + NFTs) they will create far more economic value than they could from any one game. Imagine Fortnite, but other developers can build experiences on top of the V-Bucks and skins. Epic would get a royalty every time any transaction happens. As big as Fortnite is today, Open Fortnite could be much bigger, because it will be a true platform. NFTs are better for gamers Allowing gamers to have ownership of the assets they buy and earn in game allows them to participate in the potential growth of a game. It lets gamers preserve some economic value when they switch to playing something new. But what about the criticisms of NFTs?\\
Here are my thoughts on the common FUDs: "It’s just a money grab on the part of the studios!"\\
Game studios already switched over to the model of selling in-game items, cosmetics, etc to players long ago. But currently the digital stuff players are buying isn’t re-sellable. NFT ownership is strictly better for players. "The games aren’t real games." This reminds me of the criticism of free-to-play in 2008, when the games were Mafia Wars / FarmVille. We haven’t had time for great developers to create incredible experiences yet. Everyone investing in games knows there are great teams building. "Game NFTs aren’t really decentralized because they rely on models / assets inside centralized game clients."
Crypto is as much a movement as it is a technology. Putting items on a blockchain is what gives people trust that they have participatory ownership...which make people willing to buy in to the game. These assets are “backed” by blockchain.
The fact that these item collections are NFTs will make other people willing to build on top of them. "NFTs are bad for the environment." Solana and L2s solve this. NFT games are better for players and for game developers. Like the free-to-play revolution changed gaming, so will blockchain. The games of the future will be fully robust, with open and programmable economies.}''




\label{behaviours}
\begin{itemize}
\item As a user I want to select a digital asset I find in the AR/VR world and then be offered an option to purchase the asset so I can look at it in my own spaces.
\item As a user I want to click on a digital asset I find in the AR app and be given the opportunity to buy it as a rare digital representation so that only I and a few others are provably certified to own.
\item As a user I would like to transfer economic value to people and entities I meet in the metaverse such that it is agreed by all parties quickly that value has been provably transferred.
\item As a user I would like to access an online marketplace in the metaverse where I swap and trade digital assets with other users so that I continue to feel engaged.
\item As a user I would like to create content (inside or outside of the metaverse) so I can take it to metaverse and monetise it.
\item As a content creator or influencer I would like to engage with live audiences within the metaverse, and moneytise my opinions and knowledge in real-time. I would like to have a way to split this money with co-collaborators in real time.
\end{itemize}
\section{Crypto metaverses}

\href{https://naavik.co/business-breakdowns/axie-infinity/#axie-decon=}{Report on Axie Infinity}

\href{https://www.thesun.co.uk/tech/17348918/pavia-metaverse-cardano-crypto-game/}{Pavia Metaverse}
Probably the best example in the market at this time with connecting users with one another through blockchain is \href{https://lightnite.io/}{Satoshis Games `Litenite'}. Litenite is a `battle royale' game which allows users to earn Satoshis through the Lightning network.\par
Similarly, and potentially more significantly, \href{https://twitter.com/zebedeeio/status/1512128093653196809}{Zebedee} have brought Lightning based micropayments to \href{https://zebedee.io/infuse/}{Counter Strike}, which adds a financial layer directly to eSport, itself a multi billion pound global industry.\par
The Zebedee model is interesting in that they provide simple onboarding, and management solutions, for gaming and metaverse application developers. There is doubtless an opportunity to utilise their business model in the proposed stacks in the paper, but it would be at odds with the free and open source product methodology in this paper. Their CTO said the following in a \href{https://lightningjunkies.net/lightning-address-making-lightning-user-friendly-lnj052/}{recent podcast}:\par
``We all had very similar ideas around being able to put Lightning network capabilities into games. You're essentially putting real value inside of the game. So whether it's a point inside of the game or as a real end game economy, as a game developer, you don't have to worry about the mechanics around it.\par
You can use a real life currency: the money that exists in the world and that value carries regardless of which game you're in, regardless if you're in the real world or inside of a virtual world, like a game. We just think that vision is just sort of opening. Now there's so much more, if you extrapolate it into the Meatverse we would love for Zebedee to be a big platform provider and enabler for a lot of these.''\par
\href{https://spellsofgenesis.com/}{Spells of Genesis} is a long running card RPG trading game on mobiles which allows ``ownership'' of items and cards through non-fungible token ecosystems.\par
There are also hundreds of casinos which operate within and even on blockchain networks. These feel out of scope as they are a different and somewhat regulated offering.


==> 08_metaverse_points.tex <==
\section{Summary TL;DR}
\label{sec:tldr}
\begin{itemize}
\item There may be an inflection point in the organisational topology of the internet, because of trust abuses by the incumbent providers. This moment has been calling itself Web3, but the moniker is fraught with problems, and somewhat meaningless. The drivers are real.
\item `The Metaverse' is coming, in some form, at some point. Everyone is positioning in case it's ``soon''. It's not at all clear what it is, or if people want it, but the best of the emergent narrative looks like the older field of ``digital society'' and that obviously should not be dismissed lightly.
\item Large scale `social' \& immersive metaverse is suffering poor adoption, failing as it has in the past. It's likely that the market need has been overstated. More advanced and popular (closed) games based solutions do not serve societal or business needs.
\item The closest contenders at this time are Roblox for social and `play', VRChat for more `serious' users, and Nvidia Omniverse for high end business to business metaverse.
\item From a business perspective metaverse is the worst of the remote collaboration tool-kits, and undermines flow, productivity, and interpersonal trust. Metaverse is probably technology for technologies sake at this time, but the investment is real. 
\item Digital society may be a more tangible and less hyped term to build around, and extends out into the more compelling spatial and augmented reality technologies, web, and digital money and trust.
\item Emerging markets, less developed nations, indeed much of the world is excluded from many of the tools that are taken for granted in `Western' digital society. They do not necessarily have the identification, banking rails, or compute power to engage fully. Our focus is on Africa and India.
\item Excluding Facebook/Meta, a lot of the investment is coming from the recent Web3 speculative bubble. They have a parallel and intersectional metaverse narrative, based around distributed financial tooling and digital assets. 
\item There is genuine, undeniable interest in digital scarcity. The ownership of digital goods seems natural to younger, digitally native users. This is serviced already by various (gaming) platforms, but they are all isolated ecosystems.
\item Uniting these attempts, with portable (transferable) ``goods'' across digital society likely requires a global ledger (blockchain), indeed this is the basis of the Web3 interpretation. Crypto is igniting imagination on this topic, and is seeing adoption both inside out outside of the metaverse context. There are other potential options available soon.
\item Crypto is a nightmare; rife with scams, poor technology choices, limited life, and incorrect assumptions. The only thing blockchain / crypto can do well is ``money like networks'', which is a cornerstone of human interaction, and the killer application. We strongly believe that Bitcoin is the signal, and crypto is the noise.
\item Representations of dollars and pounds can ride securely on top of such networks as stablecoins, and this is getting easier to integrate, though there are risks. This has the potential to open up global collaborative working practices, inclusive of emerging markets.
\item It's unclear which technology will win, if any, but since the tools exist now they can be integrated and tested immediately. Money, digital artefacts, identity, and thereby trust, can already be mediated by the Bitcoin network, even without using Bitcoin the asset. 
\item Legislative and cultural headwinds are significant. There might be no opportunity here in the end, though ``rough game theory'' supports the attempt.
\item Industry has noted the risk, and failures of Meta across both metaverse, and digital currency, and have latched onto "open metaverse" as a narrative, to de-risk their interest. The current open metaverse is muddy and confused. 
\item A truth seems to have been missed; that open metaverse should mean open source metaverse. There are some options, but they are under developed. We would like to contribute to this by applying our decades of telecollaboration research. 
\item The UK seems to be endorsing significant controls and restrictions on internet usage including metaverse applications. This compliance overhead will price small companies out of large scale social experiences. Company walled gardens are less impacted (as per the slack service model), and this is an opportunity if tied to real business use cases.
\item Anything from a multi-million pound XR studio screen, to a speech audio system, can be a digital society interface.
\item The newly forming Nostr protocol may be an opportunity to link and federate small and useful mixed reality spaces, providing some identity assurances, mediating data synchronisation, allowing `machine to machine' communication, while maintaining \textit{reasonably} strong cryptography throughout.
\item AI \& machine learning and especially `generative art' is further blurring these boundaries. A better term for AI/ML is `supported creativity' and/or `augmented intelligence'. While current models such as GPT3.5 and LAION based generative systems are already causing a global stir, it's likely that the soon to be released GPT4 will force global debate about general AI.
\item Trust, accessibility, governance, and safeguarding, are hard problems, and made more complex by unrecorded social flow in immersive social VR.
\item The challenge is to build a topologically flat, inclusive, permissionless, federated, and open metaverse, with economically empowered ML and AI actors, which can mediate governance issues, transparently, according to well constructed custom schemas, between cryptographically verifiable economic users (human or AI).
\item New open source [supported creativity, augmented intelligence] tooling from StabilityAI, and multiple large language models, potentially removes many of the problems with accessibility, creativity, language barriers, safeguarding, and governance. This is a huge, complex, and fast moving area, but tremendously exciting. 
\item Using new image generation ML it may be possible to build new kind of collaborative global networks for training, research, biomedical, and creative industries, ideating in simplistic immersive spaces while instantly creating scenes which can be stylised using verbal commands in real-time. This may open up and enfranchise fresh ideas from a wider cultural pool.
\item Such teams could could be far more ad-hoc by experimenting with the designs outlined in this book. This kind of genuine digital society use case is something sorely lacking in large scale attempts such as Meta Horizons. It need not be complex or large scale, but it must be secure, trusted, and task appropriate. We think we can deliver this and conversations with the industry suggest that there is excitement and cautious appetite. 
\end{itemize}



==> 09_LLMs.tex <==

\section{Overview of Large Language Models}
In the last year or two it's become obvious to most people that ``artificial intelligence'' is intuitively and subjectively real for the first time. Around half of adults in the west are now aware of ChatGPT. To be clear AI is still a pretty meaningless term. `Intelligence' is one of those slippery words which is highly dependent on context. A satnav system running on a phone can make an intelligent choice about a route by synthesising data and presenting comprehensible results, but it seems absurd to ascribe an intelligence to it. It's possible that there's some kind of ``spoooky'' quantum activity in play in a conscious human brain, as described in mind bending mathematical depth by Penrose in 1989 \cite{penrose1990emperor}. It's something of an unknown unknown \cite{kerskens2022experimental}, and that we'll never get to what's called `strong' or `general' AI \cite{larson2021myth, searle1980minds}, reserved by some scientists for ``true consciousness'', whatever that means. With that said we may be approaching the threshold of the `Turing Test` \cite{sep-turing-test}, initially posited by Alan Turing in 1950 \cite{turing1950computing}, and the goalposts have begun to move in response to claims that there have been successful examples \cite{warwick2016can, french2012moving, french2000turing, searle2009turing}. It feels that in this moment it is appropriate to open with an ethics section.\par
To set the tone here let's have OpenAI's ChatGPT give us a definition:
\begin{tcolorbox}[enhanced, frame style={fill=lightgray}, interior style={fill=lightgray}]Intelligence is the ability to acquire and apply knowledge and skills in order to solve problems and adapt to new situations. It can involve a range of cognitive abilities, such as perception, learning, memory, reasoning, and decision-making. Intelligence is a complex and multifaceted concept that has been studied by psychologists, philosophers, and scientists for centuries.
\end{tcolorbox}
The Oxford English Dictionary defines Artificial intelligence as 
\begin{tcolorbox}[enhanced, frame style={fill=lightgray}, interior style={fill=lightgray}]The capacity of computers or other machines to exhibit or simulate intelligent behaviour''.
\end{tcolorbox} 
This is very murky territory. The boundary line between very capable trained systems and something that \textit{feels} like intelligence is obviously a subjective one, and different for each person and context, (Figure \ref{fig:aiVenn}).\par

\begin{figure}[ht]\centering 	\includegraphics[width=0.8\textwidth]{ai}
	\caption{The terminology in the field is both somewhat blurred and highly `nested'.}
	\label{fig:aiVenn}
\end{figure}

I will use AI and ML interchangeably in this text, but in so doing I hope to draw attention to the moment we find ourselves in. It feels like there is an inflection point in human history happening right now, with AI as a cultural truism and the more honest `machine learning' relegated to history. \par
Irrespective of the gap between the perception and truth around these systems there is now a feedback loop where the data that these systems are trained on will be learning from both human \textbf{and} outputs from such systems, to the detriment of both models and humans\cite{shumailov2023curse}. Today's young children will never know a world in which the information they encounter is verifiable as of purely human origin. The implications of this are unclear but exciting. \par
In the field of natural language processing, there have been significant advancements in the use of language models for various tasks. These models are trained on large amounts of text data and are able to generate coherent sentences or paragraphs. They have been used for tasks such as language translation, text summarization, and sentiment analysis. GPT3 and GPT4 are the most widely known examples, and are right in the boundary space where ML begins to look like AI. To be clear such language models are many layers short of AI \cite{elkins2020can, marcus2020gpt}. We have by now all seen these work but here's a quick comparison demonstrating the rate of change. The following was fed into ChatGPT 3.5: ``write a poem in iambic pentameter about the difficulty humans have deciding if a thing is really intelligent.''
\newpage
\begin{tcolorbox}[enhanced, frame style={fill=lightgray}, interior style={fill=lightgray}]``Is it true intelligence, or just a guise?
We struggle to decide with troubled brow
For machines can mimic, with clever guise
The way we think and work, with nimble now
But do they truly understand and feel?
Or is it just a programmed façade?
We ponder on this question, with a zeal
For understanding if intelligence is a nod
To mere programming, or something more profound
A spark of consciousness, a self-aware mind
These questions plague us, yet we are not bound
By any one answer, we are free to find
Our own conclusion, as we ponder and muse
On the true nature of intelligence and its use''.
\end{tcolorbox}

This is the GPT4 version a month later, handling the LaTeX formatting itself:\\

\itshape{
Upon the realm of mind and cogitation, \\
A question looms with great anticipation. \\
Doth sentient life in circuitry exist, \\
Or is it but a dream, a wisp of mist? \\

In measured beats of thought, the heart doth race, \\
As human minds grapple with cyberspace. \\
When metal minds in cold precision speak, \\
Do we, in truth, behold intelligence unique? \\

From Turing's test, the doubts and queries sprout, \\
A test to quell the din of skeptic's shout. \\
Yet do these trials prove with certainty, \\
The depth of thought, the spark of liberty? \\

Alas, we seek a scale, a touchstone pure, \\
To judge the essence of the mind obscure. \\
But in that quest, we find ourselves confound, \\
For truth, like wind, doth ever shift around. \\

The line between machine and man doth blur, \\
As thoughts entwined, a tangled web they stir. \\
To tell apart the spirit from the gears, \\
We strain our eyes, confront our deepest fears. \\

In iambic verse, we search the bounds of thought, \\
To wrest the truth from shadows, ever sought. \\
But answers true remain elusive still, \\
The more we grasp, the more they slip our will. \\

For in this dance, intelligence doth sway, \\
And human hearts, beguiled, are led astray. \\
To judge the spark within the wires and code, \\
We must look inward, seek our own abode.}
\normalfont


\subsection{How they work}
For an excellent youtube video on the subject I would currently recommend \href{}{this presentation} from OpenAI founder Andrej Karpathy. Their system is the GPT3-4 series that everyone is familiar with, and the first few sections will concentrate on those options. If you know this stuff you can skip to section \ref{sec:llmoptions}. Alternatively if you want more then you can head to the appendix \ref{sec:aiterms} to see where I am up to in my learning, or else dive straight into the Little Book of Deep Learning \cite{fleuret2023little}. \par
All these systems run \textbf{purely} on numbers. The input data that they are trained on are compressed enormously into a thing called latent space \cite{DBLP:journals/corr/abs-2112-04895}, which is `loosely analogous' to a massive cloud of numbers. The text you type into interface is chopped up into ``tokens'', which is a leftover word from natural language processing research. Tokens are numbers that match words, or bits of words. This varies a lot depending on the techniques being used, but for our purposes we simply need to know that all the words you input, become somewhat \textit{more} number representations, which are then fired off into the latent space number cloud to find patterns that kinda match. This input is usually refered to as the `context window', or `token limit'. In GPT4 it's 8000 tokens (6000 words) and in GPT3.5 Turbo it's 16,000 tokens.  What comes back out of the cloud is statistically most likely sets of numbers which flow from the end of the enormous number input. Polymath and general all round genius Stephen Wolfram explains all this very well \href{https://writings.stephenwolfram.com/2023/02/what-is-chatgpt-doing-and-why-does-it-work/}{in a blog post}.\par
LLMs simply take whatever is in front of them and ``try to complete the document'' using their vast store of ``things that look like this document''. When you are chatting with them there's a bunch of contextual stuff pre-loaded onto the text you type. You don't see this input go in, but it sets up the broader document which the big autocomplete is tasked with finishing. This is ``very roughly'' of the context:
\begin{tcolorbox}[enhanced, frame style={fill=lightgray}, interior style={fill=lightgray}]
``Below is an instruction that describes a task, paired with an input that provides further context. Write a response that appropriately completes the request.

--- Instruction:
Instruction

--- Input:
Input

--- Response:''
\end{tcolorbox}
As the conversation with the chat interface continues the users' prior inputs are added into the context, and that goes in with each and every request. This builds up quickly to reinforce the current conversational flow. The model is inherently blind to the previous conversations, it's just being fed more and more of the previous chat behind whatever you just typed. This is where the systems currently break down. The input frame for ChatGPT is generally 8000 tokens. This allows a lot of chat (about 6000 words), but anyone who's used these systems will have seen it `forget' the earliest context as those tokens fall out of the back of the input frame.\par 
\subsection{Evolving Landscape of LLM Pipelines}

This section delves into the key pillars that form the backbone of deploying and managing these advanced systems.

\begin{comment}
flowchart TB
    A[Start: User Request] -->|Determine Jurisdiction| B[Jurisdiction Check]
    B -->|Data Input| C[Observability]
    C --> D[AI Gateway]
    D -->|Model Selection| E[Model Interaction]
    E --> F[Security and Compliance Check]
    F --> G[End: Deliver Response]

\end{comment}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.2\textwidth]{llmflow}
    \caption{The flow of data through a modern LLM pipeline}
    \label{fig:llmflow}
\end{figure}



\subsubsection{Observability in AI Systems}
Observability plays a pivotal role in the effective management of AI and LLM pipelines. It involves a comprehensive monitoring mechanism that encompasses various aspects:
\begin{itemize}
    \item \textit{Performance Monitoring:} Tracking the efficiency and accuracy of AI models in real-time.
    \item \textit{System Health Checks:} Regular assessments to ensure the AI systems are functioning optimally.
    \item \textit{User Interaction Analysis:} Understanding how users interact with AI systems to enhance user experience.
\end{itemize}

\subsubsection{The AI Gateway: A Multiplex Interface}
The AI Gateway acts as a central hub, orchestrating the interaction between different AI models and the user interface. Key functionalities include:
\begin{itemize}
    \item \textit{Model Integration:} Seamlessly connecting various AI models to the system.
    \item \textit{Dynamic Swapping:} Allowing for the exchange of models without disrupting the system’s operations.
    \item \textit{Load Balancing:} Distributing requests effectively among different models to optimize performance.
\end{itemize}

\subsubsection{Prompt Management and Experimentation}
Effective communication with AI models is achieved through carefully crafted prompts. This area focuses on:
\begin{itemize}
    \item \textit{Prompt Library Development:} Creating a diverse range of prompts to elicit specific responses from AI models.
    \item \textit{A/B Testing:} Experimenting with different prompts to determine the most effective ones.
    \item \textit{User-Centric Design:} Tailoring prompts to align with user preferences and behaviors.
\end{itemize}

\subsubsection{Security and Compliance in AI Ecosystems}
Ensuring the security and regulatory compliance of AI systems is crucial. This involves:
\begin{itemize}
    \item \textit{Data Privacy Measures:} Implementing strategies to protect sensitive user data.
    \item \textit{Regulatory Compliance:} Adhering to global standards and regulations like GDPR (including segmentation of personal data and routing issues).
    \item \textit{Threat Mitigation:} Developing robust defences against cyber threats and vulnerabilities.
\end{itemize}

Each pillar represents an integral component in the architecture of modern AI and LLM pipelines, facilitating their evolution and adaptation in a fast-paced digital world.

\subsection{Ethics \& Impact}
AI ethics is now a hot topic even outside of the academic fields which have previously wrestled with these issues. These new systems are thought likely to be able to impact all human activity \cite{eloundou2023gpts}. \par
The Centre for Humane Technology \href{https://www.humanetech.com/key-issues}{highlight the negative assessment} of the risk of Large Language Models, stating that major advancements in AI are coming and society needs to address the issues before they become `entangled'. The misalignment problem with social media has not been fixed, and this is where Harris and Raskin made their name. Their focus is not on AGI apocalypse scenarios but rather on the potential consequences of rapid AI advancements. AI has evolved significantly since 2017. They somewhat hyperbolically call such models `golems', in reference to their emergent capabilities. They would like society to address the potential risks of LLMs before they become entangled in society and to better understand and manage their impact.\par
They highlight author \cite{harari2014sapiens} Harari's quote: \textit{``What nukes are to the physical world, AI is to the virtual and symbolic world.''} - and this quote feels very compelling when held up against our assertions about cryptographic end points and trust.\par
Rosenburg describes \href{https://bigthink.com/the-present/danger-conversational-ai/}{`The AI manipulation problem'} which refers to the emerging risk of real-time engagement between a user and an AI system that can impart targeted influence, sense the user's reactions, and adjust tactics to maximize persuasive impact. This can occur through natural spoken interactions with photorealistic virtual spokespeople that look, move, and express like real people. Conversational AI can push individual emotional buttons by adapting to personal data and analyzing real-time emotional reactions, becoming more skilled at playing each user over time. This presents a serious concern as it can be used to influence individuals and broad populations in ways that may be damaging to society \cite{Rosenberg2023}. \par
As AI models improve, they are generating their own data for reinforcement learning, with humans only needed to train the reward function. The advancements are not limited to algorithms and APIs; even hardware is advancing rapidly due to AI, as shown by Nvidia's research on using AI to improve chip design.\par
GPT-4 is breaking its \href{https://nanothoughts.substack.com/p/reflecting-on-reflexion}{own records} through self-reflection. This reflection paper has caught global attention and shows GPT-4's ability to improve upon its mistakes, and enhance its performance in a variety of tasks \cite{shinn2023reflexion}. The process of self-reflection has been observed in other research papers as well, demonstrating its effectiveness in improving model outputs.\par
The groundbreaking Huggingface GPT model can draw upon thousands of other AI models to perform tasks involving text, image, video, and question answering \cite{shen2023hugginggpt}. The Hugging GPT paper reveals a model that can connect numerous AI models for solving complex tasks, using language as an interface. It can perform tasks such as describing and counting objects in a picture, generating images and videos, deciphering invoices, and even describing them in perfectly simulated human voices.\par
The rapid advancements in AI are causing commercial pressure, pushing companies like Google to catch up with the likes of OpenAI. With self-improvement, tool use, hardware advances, and commercial pressure, the future of AI seems to be on a trajectory of rapid growth and development. The most recent comparator is the emergence of the iPhone and death of Adobe Flash \cite{horton2019death}, but this is orders of magnitude beyond that and likely most analogous to the industrial revolution \cite{trajtenberg2018ai}. \par 
\href{https://www.key4biz.it/wp-content/uploads/2023/03/Global-Economics-Analyst_-The-Potentially-Large-Effects-of-Artificial-Intelligence-on-Economic-Growth-Briggs_Kodnani.pdf}{A Goldman report} sees 25\% of roles basically wiped out. Even OpenAI themselves published similar findings \cite{eloundou2023gpts}. The systems can already pass almost all human examinations with ease, causing immediate existential harm to education assessment systems.\par 
The risks of generative AI are well covered by a \href{https://www.citizen.org/article/sorry-in-advance-generative-ai-artificial-intellligence-chatgpt-report/}{Public Citizen article}, and are simply listed below to get us started. It is a huge and well researched report and this list doesn't do it justice:
\begin{itemize}
\item A sharp increase in political disinformation;
\item Intensified, widespread consumer and financial fraud;
\item Intrusive privacy violations beyond those already normalized by Big Tech;
\item Harmful health impacts, from promotion of quack remedies to therapeutic malpractice;
\item Amplification of racist ideas and campaigns;
\item Destruction of livelihoods for creators;
\item Serious environmental harm stemming from generative A.I.’s intense energy usage;
\item The stripping of the information commons;
\item Subversion of the open internet;
\item Concentration of economic, political, and cultural power among the tiny number of giant companies with the resources to develop and deploy generative A.I. tools.
\end{itemize}

Research suggests that LLM outputs cannot be discriminated from human output in meaningful ways, casting shade across all assessed measures of humans in written form \cite{sadasivan2023can} from this point forward. Michal Zalewski \href{https://lcamtuf.substack.com/p/llms-a-bleak-future-ahead}{says}: \textit{``Instead of taking sides in that debate, I’d like to make a simpler prediction about LLMs as they operate today. I suspect that barring urgent intervention, within two decades, most of interactions on the internet will be fake. It might seem like an oddly specific claim, but there are powerful incentives to use LLMs to generate inauthentic content on an unprecedented scale — and there are no technical defenses in sight. Further, one of the most plausible beneficial uses of LLMs might have the side effect of discouraging the creation of new organic content on the internet.''}

Within generative machine learning there has been a raging debate between `some' of the artists whose original works were `scraped' into the \href{https://laion.ai/}{LAION} open dataset. Far more can and should be said on this, but I suspect Immersive has it's own advanced opinions so I won't attempt to cut across them.\par
AI safety and the challenges associated with managing an AI system's output are important considerations. Efforts have been made to ensure AI safety over the years, but the pace of change may be outstripping the ability of the industry and researcher to keep up. Finding the right balance between allowing users to express themselves and drawing the line on harmful or offensive content is a difficult task. Defining concepts like hate speech and harmful output, as well as aligning AI systems with human values and preferences, are complex challenges. Ideally, a democratic process would involve people from different perspectives coming together to decide on rules and boundaries for AI systems. However, implementing such a process is not straightforward, and developers must remain heavily involved in decision-making while still seeking input from a broader audience.\par
It is beyond the scope of this text to dig far into these issues, but they have serious implications for anyone working in the space. \par 
\subsubsection{AI's lying heart}
Large language model systems, at this time, are given to making things up. They `hallucinate' very cogently \cite{azamfirei2023large}, presenting completely erroneous assertions and data as facts, with \href{https://news.artnet.com/art-world/chatgpt-art-theory-hal-foster-2263711}{figures to back them up}. Perhaps counter intuitively this problem extends into pure mathematical realms, with seemingly simple arithmetic causing the systems problems. Both of these are the same problem, the models descend the most statically plausible path toward an output based pretty much on the last character generated along the vector into the n dimensional algebra space. This is being ameliorated through self checking \cite{manakul2023selfcheckgpt}, human reinforcement learning \cite{ouyang2022training}, and integration of specialised tools \href{https://writings.stephenwolfram.com/2023/01/wolframalpha-as-the-way-to-bring-computational-knowledge-superpowers-to-chatgpt/}{like Wolfram Alpha}, behind the models.\par 
Media outlets such as The Guardian are rushing to publish open guidelines on \href{https://www.theguardian.com/commentisfree/2023/apr/06/ai-chatgpt-guardian-technology-risks-fake-article?}{how they intend to deal} with the problem of GPT based article research, and it seems that \href{https://www.bbc.co.uk/news/technology-65202597}{legal challenges} will quickly mount up. With that said, the UK government is currently signalling a \href{https://www.gov.uk/government/publications/ai-regulation-a-pro-innovation-approach}{``pro-innovation''}, hands off approach to AI, and is \href{https://www.gov.uk/government/news/initial-100-million-for-expert-taskforce-to-help-uk-build-and-adopt-next-generation-of-safe-ai}{investing significantly} in supporting the technology.
\subsubsection{Alignment and take-off of AGI}
AI has the potential to significantly improve quality of life, but it is essential to ensure that it remains aligned with human values and does not harm or limit humanity. Alignment in language models trys to address this by incorporating strategies, which can be broadly categorized into the following areas:
\begin{itemize}
\item \textbf{Pre-training} In the initial stage, models are trained on a large dataset containing diverse text from the internet. This allows them to learn grammar, facts, reasoning abilities, and some level of world knowledge. However, they can also learn biases present in the data. Alignment efforts at this stage may involve dataset choices, monitoring, and some feedback to reduce reduce obvious biases.
\item \textbf{Fine-tuning} After pre-training, models are fine-tuned on a narrower, more specific dataset, often with human-generated examples and labels. During fine-tuning, alignment efforts can include generating clearer instructions for human reviewers, providing them with guidelines and feedback, and iteratively refining the process to improve the model's behaviour. Things like ranked lists of responses from the system would go in this stage. This is the ``human reinforcement learning'' which has so invigorated LLMs recently \cite{perez2022discovering}.
\item \textbf{Evaluation} Assessing the performance and safety of a language model is crucial for alignment. This can involve creating evaluation metrics, benchmarks, and tests to measure the model's progress in terms of safety, usefulness, and alignment with human values. Some of these are encoded inline with the model generation and are called `hyperparameters'. Two important hyperparameters that influence the generated text are frequency penalty and presence penalty. Frequency penalty affects the repetition of tokens in the generated text by modulating the probability distribution of tokens. A positive frequency penalty value discourages the model from choosing frequently occurring tokens, leading to a more diverse and sophisticated vocabulary. Presence penalty influences the generation of tokens that have already appeared in the generated text. A higher presence penalty value discourages the model from repeating tokens or phrases, ensuring a more cohesive and engaging output. On the other hand, a lower presence penalty value allows the model to generate text with repeated tokens or phrases, which can lead to redundancy and reduce the overall coherence of the text.\par 
So called use of `Red Teams' goes in this section, but much of this has recently been done live on alpha and beta public testing. 
\item \textbf{Safety mitigations} Addressing risks associated with harmful outputs, non-consensual content, and other safety concerns is an essential aspect of alignment. Techniques like more reinforcement learning from human feedback, rule-based filters, and output constraints can be employed to reduce harmful outputs and improve model safety. These feedback loops at the end of the process carry a disproportionate weight in the models, and it is at this stage that the most noticeable change is sometimes introduced. It is critical to get the maximum global public engagement during this final feedback into the system, from policy-makers and diverse human response feedback. It's not clear this is yet happening. Even Altman, the CEO of OpenAI admits that the models likely reflect the training choices of San Francisco `Tech Bros' in this moment. That is clearly not good enough.
\end{itemize}
Altman, says they have optimised their approach based on aiming for earlier AGI, but a slow AGI "takeoff", ie, the dfference between a gradual understandable creep toward a general intelligence, vs "AI FOOM" \cite{yudkowsky2008hanson}. They have a weighted risk matrix, but no clear ideal -yet- as to what the tools look like to keep the AGI "aligned" with humanity. Starting fast, but asserting slow and steady about the emergent behaviour part seems optimistic at best. Nonetheless this is likely the best/only approach, assuming it' possible. The only alternative is literally the ``Butlerian Jihad'' from Herberts' Sci-Fi DUNE.\cite{song2018preventing}.\par
There is a possibility that AI could become misaligned as it gains superintelligence, and it is essential to acknowledge and address this risk. 
AI technology, such as GPT-4, has shown exponential improvement, raising concerns about AI takeoff, which could happen rapidly within days. While GPT-4's performance has not been surprising to some, its impact highlights the need to increase technical alignment work and continually update the understanding of AI safety.\par
It's noteworthy that industry luminaries such as Yoshua Bengio, Turing Prize winner, Stuart Russell, director of the Center for Intelligent Systems, Elon Musk, and Steve Wozniak, Co-founder of Apple co-signed an \href{https://futureoflife.org/open-letter/pause-giant-ai-experiments/}{open letter} requesting a 6 month pause on the development of these systems. For what it's worth I have also signed. The narrative needs time to catch up. To be clear it won't happen, but the signalling here is part of building the awareness that is sorely lacking. 
\subsubsection{Industry capture, and failure to democratise}
Financial time article, integrate:
\begin{tcolorbox}[enhanced, frame style={fill=lightgray}, interior style={fill=lightgray}]``There's a colossal shift going on in artificial intelligence - but it's not the one some may think. While advanced language-generating systems and chatbots have dominated news headlines, private AI companies have quietly entrenched their power. Recent developments mean that a handful of individuals and corporations now control much of the resources and knowledge in the sector - and will ultimately shape its impact on our collective future. The phenomenon, which AI experts refer to as "industrial capture", was quantified in a paper published by researchers from the Massachusetts Institute of Technology in the journal Science earlier this month, calling on policymakers to pay closer attention. Its data is increasingly crucial. Generative AI - the technology underlying the likes of ChatGPT - is being embedded into software used by billions of people, such as Microsoft Office, Google Docs and Gmail. And businesses from law firms to the media and educational institutions are being upended by its introduction.
The MIT research found that almost 70 per cent of AI PhDs went to work for companies in 2020, compared to 21 per cent in 2004. Similarly, there was an eightfold increase in faculty being hired into AI companies since 2006, far faster than the overall increase in computer science research faculty. "Many of the researchers we spoke to had abandoned certain research trajectories because they feel they cannot compete with industry - they simply don't have the compute or the engineering talent," said Nur Ahmed, author of the Science paper. In particular, he said that academics were unable to build large language models like GPT-4, a type of AI software that generates plausible and detailed text by predicting the next word in a sentence with high accuracy. The technique requires enormous amounts of data and computing power that primarily only large technology companies like Google, Microsoft and Amazon have access to. Ahmed found that companies' share of the biggest AI models has gone from 11 per cent in 2010 to 96 per cent in 2021. A lack of access means researchers cannot replicate the models built in corporate labs, and can therefore neither probe nor audit them for potential harms and biases very easily. The paper's data also showed a significant disparity between public and private investment into Al technology. In 2021, non-defence US government agencies allocated \$1.5bn to AI. The European Commission planned to spend \$1.5bn. Meanwhile, the private sector invested more than \$340bn on Al in 2021.''
\end{tcolorbox}
\subsubsection{Cybersecurity implications}
It seems clear to all observers of the potential LLMs to be leveraged in supranational misinformation campaigns, zero-day exploits, and other geopolitical threats. It's appropriate to contextualise American export restrictions on powerful GPU and TPU hardware to China and Iran, and the implications of LLMs being "in the wild" and easily retrained for nefarious purposes. These powerful tools can be weaponised by malicious actors to create a new frontier of cybersecurity threats. 
\begin{itemize}
\item Supranational Misinformation Campaigns: 
LLMs can be easily retrained and used to generate convincing disinformation, thereby escalating the effectiveness of misinformation campaigns. As LLMs become more accessible, nation-states and non-state actors can utilise these technologies to create more targeted, sophisticated, and persuasive disinformation. This could lead to widespread confusion and mistrust, ultimately undermining the credibility of institutions and weakening social cohesion.
\item Zero-Day Exploits: 
Aggressive state actors can exploit LLMs to discover and leverage zero-day vulnerabilities. By training LLMs on massive amounts of data related to software development, vulnerabilities, and exploits, malicious actors can potentially identify previously unknown weaknesses in critical systems. These actors could then launch devastating cyberattacks, causing significant damage to their adversaries' infrastructure, economy, and security.
\item Autonomous Incursions:  Highly Compressed LLMs can potentially deploy autonomous incursion suites like Stuxnet, but with a greater degree of autonomy and less reliance on command and control. These advanced incursion suites might infiltrate targeted systems, adapt to their environment, and blend in with legitimate traffic, making them difficult to detect and mitigate. The integration of LLMs into these suites increases the potential for damage and disruption.
\end{itemize}
In response to these threats, the United States has imposed export restrictions on powerful GPU and TPU hardware to China. While these restrictions may slow down the development and deployment of LLMs for malicious purposes, they are unlikely to provide a long-term solution. As LLMs become more accessible and the technology proliferates, bad actors will trivially acquire the necessary hardware through alternative means, and the model weights themselves are already freely available. Existing defenses may not be adequate to counter the threats posed by LLMs, and the development of new cybersecurity measures requires time, resources, and expertise. In the absence of substantial increases in cybersecurity investment and research, it is likely that adversaries will continue to exploit LLMs to their advantage.\par
\href{https://securityintelligence.com/news/are-threat-actors-using-chatgpt-to-hack-your-network/}{According to Brad Hong}, Customer Success Manager with Horizon 3 AI, ``attackers are likely to adopt code generative AI as a means to address their limitations in scripting skills.'' Hong explains that code generative AI acts as a bridge, translating between languages that the attacker may not be proficient in and providing a means of generating base templates of relevant code. This reduces the skill requirements needed to launch a successful attack, as it serves as a tool in the attacker's arsenal alongside other tools.\par
In an email interview, Hong notes that the use of code generative AI, such as chat GPT, supercharges the attacker's ability to launch successful attacks. As explained by Patrick Harr, CEO at SlashNext, in an email comment, said \textit{``ChatGPT enables threat actors to modify their attacks in millions of different ways in minutes, and with automation, deliver these attacks quickly to improve compromise success.''}\par
The developers of chat GPT were aware that threat actors would attempt to weaponize the AI. As Harr explains, ``hackers are really good at weaponizing whatever technology is put in front of them.'' To mitigate this risk, the developers implemented preventive measures, such as flagging certain words and terms, like `ransom' or `ransomware.' For example, when researchers at Deep Instinct typed in the word `keylogger,' the chatbot responded with ``I'm sorry but it would not be appropriate or ethical for me to help you write a keylogger.''\par
However, these restrictions can be circumvented with a bit of clever rewording. As Jared, a Competitive Intelligence Analyst with Deep Instinct, explains, ``there's always a workaround.'' For example, instead of asking chat GPT to create ransomware code, an attacker could request a script that encrypts files and directories, drops a text file into the directory, and subdirectories.\par
The ability to weaponize chat GPT, or any other AI chatbot, is a game-changer for threat actors. With the ability to modify malicious code quickly and bypass cybersecurity defenses, these tools have the potential to greatly increase the effectiveness of attacks. As such, it is important for cybersecurity professionals to stay informed about the evolving threat landscape and the tools and techniques used by attackers \cite{brundage2018malicious}.\par 
At this early stage in the technology it is important that corporate and private users alike bear in mind that the LLMs are `leaky' and are using the data fed into them to train themselves. They are \href{https://help.openai.com/en/articles/6783457-chatgpt-general-faq}{explicit about this}. Anything that goes into chatGPT can resurface, as Samsung have found out \href{https://cybernews.com/news/chatgpt-samsung-data-leak/}{to their cost}.
\subsubsection{Use in war}
In the sphere of military, geopolitical, and civil defence the application of these tools is both shadowy and seemingly \href{https://www.vox.com/recode/23507236/inside-disruption-rebellion-defense-washington-connected-military-tech-startup}{somewhat incompetent}. It is an especially twisted irony that `Rebellion Defence'' seem to have modelled themselves on the rebellion movement in the Star Wars fictional universe, seemingly unaware that Lucas most likely saw the USA as analogous to the Empire in the films \cite{immerwahr202221}. A \href{https://www.stopkillerrobots.org/wp-content/uploads/2022/10/ADR-Artificial-intelligence-and-automated-decisions-Single-View.pdf}{recent report} from ``Stop Killer Robots'' identifies the governance concerns which they have been monitoring for years. They identify areas of specific concern.
\begin{itemize}
\item transparency and explainability \item responsibility and  accountability
\item bias and discrimination.
\end{itemize}
\href{https://vframe.io/9n235/}{munition detection}  and autonomous war robots to do
\subsubsection{Existential Threat}
Many serious researcher are now sounding the alarm at the speed of development. In this moment is seems likely that ascribing emergent behaviours to large language models is a mirage born of the desires of the somewhat accelerationist community, and their more moderate couterparts \cite{schaeffer2023emergent}. There is potentially competitive advantage in mandating a `slowdown' in the technology development if the company and research team you work for find themselves behind. It's hard to tell what's going on. With that said the increase over time of noise generated by fancy autocomplete, vs human signal will doubtless lead (mathematically) to an undoing of current digital society, in the end. This is already impacting the training of new LLM models \cite{shumailov2023curse}. All of that is without considering the wilder theories such as the so called `paperclip miximiser' \cite{bostrom2003ethical}
or what Yudkowsky calls the \href{https://www.lesswrong.com/tag/squiggle-maximizer-formerly-paperclip-maximizer}{``squiggle maximiser''}, a literal end of life scenario.
\subsubsection{Scaling challenges}
In the DeepMind paper that introduced Chinchilla \cite{hoffmann2022empirical} several problems with scaling were highlighted. These finding are being challenged as cleaner data shows improved results.
\begin{itemize}
\item Data, rather than model size, is currently the primary constraint on language modeling performance.
\item Large models (e.g., with 500B parameters or more) are not necessary if enough data can be leveraged.
\item Encountering barriers to data scaling would be a significant loss compared to the potential performance gains.
\item The amount of text data available for training is unclear, and there may be a shortage of general-domain data.
\item Specialized domains, such as code, have limited data compared to the potential gains if more data were available.
\end{itemize}
They argue that researchers often focus on scaling up the number of parameters rather than increasing the amount and diversity of training data. This focus on scaling numbers has led to a lack of clarity and rigour in describing the data collection processes and sources used in training these models. It seems  there are challenges associated with increasing the amount of training data, particularly in terms of quality and the diminishing returns of data scaling. As these barriers are better usderstood so does the community respond with new techniques to process the training data. The outstanding Falcon model simply parsed HTML, removed duplication, and applied so basic filtering to the `common crawl' dataset \cite{penedo2023refinedweb}. Similarly Microsoft created and incredibly efficient code support LLM trained in a matter of hours by using high quality textbooks \cite{gunasekar2023textbooks}.
\begin{itemize}
\item Generated tokens from 3 TB collection of code and text from StackOverflow
\item GPT-3.5 was used to generate 1B tokens of text similar to textbooks in the field
\item Over several days trained a small 1.3B parameter model (phi-1)
\item Used GPT-3.5 to generate text similar to the textbook exercises
\item Fine-tuned the phi-1 on the exercises
\end{itemize} 
The future is clearly not in \textit{more} but rather \textit{better} data. The most up-to-date analysis of scaling complexity is by Kaddour et al. and is well summarised by Anthony Alcaraz \href{https://www.linkedin.com/posts/anthony-alcaraz-b80763155_this-paper-is-a-must-read-for-those-interested-activity-7087728440300158976-wa_f?}{on LinkedIn} \cite{kaddour2023challenges}
 
\subsubsection{Model Design Challenges}

\begin{itemize}

\item Unfathomable Datasets
\begin{itemize}
\item Unable to thoroughly review or audit massive datasets. Leads to issues like benchmark contamination, privacy leaks, and suboptimal domain mixtures.

\end{itemize}

\item Tokenizer-Reliance
\begin{itemize}
\item Tokenizers have drawbacks like computational overhead, language dependence, and information loss.
\end{itemize}

\item Fine-Tuning Overhead
\begin{itemize}
\item Fine-tuning entire LLMs requires prohibitive compute resources and memory.
\item Obviously Low Rank Adaption (LoRA) is currently pushing the field forward in that regard.
\end{itemize}

\end{itemize}

\subsubsection{Model Behavior Challenges}

\begin{itemize}

\item Prompt Brittleness
\begin{itemize}
\item Small syntactic prompt variations can drastically change outputs. Lack of prompt robustness.
\end{itemize}

\item Hallucinations
\begin{itemize}

\item Models generate convincing but incorrect or underdetermined outputs.
\end{itemize}

\item Misaligned Behavior
\begin{itemize}
\item Outputs often poorly aligned with human values, intentions, and expectations.
\end{itemize}

\item Outdated Knowledge
\begin{itemize}
\item Pre-trained knowledge becomes inaccurate over time. Isolated updates remain difficult.
\end{itemize}

\end{itemize}

\subsubsection{Scientific Challenges}

\begin{itemize}

\item Brittle Evaluations
\begin{itemize}
\item Benchmarks are sensitive to small prompt variations. Static human evaluations become outdated.
\end{itemize}

\item Lacking Experimental Designs
\begin{itemize}

\item Papers lack controlled experiments and ablations. Vast hyperparameter space is under-explored.
\end{itemize}

\item Lack of Reproducibility
\begin{itemize}
\item Nondeterminism in parallelized training and blackbox APIs hinders reproducibility.
\end{itemize}

\item Tasks Not Solvable by Scale
\begin{itemize}
\item Some reasoning and generalization tasks exhibit inverse scaling or disproportionate memorization.

\end{itemize}

\end{itemize}
\subsection{A more optimistic interpretation}
It's possible that in a post-social media world where AI assistants become ubiquitous, there is a shift toward more meaningful human-human interpersonal relationships. If everyone has an AI assistant in their ear to help mediate their personal fears and anxieties, then we can perhaps see a path to more positive and local ways to communicate and engage with one another. The presence of AI assistants could conceivably help individuals become better listeners, communicators; ironically more empathetic. By providing personalized support and guidance, AI assistants might help us to better understand our own emotions and reactions, which in turn can lead to more authentic human interactions. If this new technology can undo the damage wrought by social media, and help us navigate our insecurities and anxieties, we may see a decline in the superficiality that has become synonymous with online interactions. This shift could lead to the resurgence of face-to-face conversations and the revitalization of community bonds, as individuals seek more authentic connections with those around them. This is still a worthwhile digital society, so long as the algorithm fuelled polarity fostered in the current is not repeated with weaponised AI assistants. AI assistants may seem less judgemental, and might promote mindfulness of our own biases and preconceptions, allowing us to approach conversations with an open mind and a willingness to learn from others. In this future, AI assistants not only serve as personal coaches and mediators for our individual fears and anxieties but also become catalysts for promoting healthier and more authentic human connections. By supporting our emotional well-being and helping us navigate interpersonal relationships, AI has the potential to transform the way we engage with one another. 
\newpage
\subsection{The Law (not a lawyer!)}
The \href{https://www.holisticai.com/papers/the-state-of-ai-regulations-in-2023}{world}, and more urgently the EU, is starting to frame it's legislative landscape one these technologies:
The USA has published it's ``AI Bill of Human Rights'', highlighting five themes:
\begin{itemize}
\item Safe and Effective Systems
\item Algorithmic Discrimination Protections
\item Data Privacy
\item Notice and Explanation
\item Human Alternatives, Consideration, and Fallback
\end{itemize}
It would be worth digging into these further here were it not so clear that the guardrails have already been breeched. The \href{https://www.whitehouse.gov/wp-content/uploads/2022/10/Blueprint-for-an-AI-Bill-of-Rights.pdf}{full report} is still worth reading.\par

\subsubsection{AI Regulation and Compliance: Navigating the Evolving Landscape}

The global urgency to regulate AI is intensifying, prompting organizations to adapt their governance structures to current and upcoming regulatory requirements. This section provides an overview of existing and new AI regulations in the EU and US, and suggests key action points for navigating AI compliance.

\paragraph{International Soft-Law Approaches}
\begin{itemize}
\item Various international bodies have adopted non-binding guidelines for ethical and responsible AI use. These include the \href{https://oecd.ai/en/ai-principles}{OECD AI Principles}, the \href{https://www.unesco.org/en/artificial-intelligence/recommendation-ethics}{UNESCO’s Recommendation on the Ethics of AI}, and the \href{https://www.whitehouse.gov/ostp/ai-bill-of-rights/}{White House Blueprint for an AI Bill of Rights}.
\item Standardization bodies such as \href{https://www.iso.org/standard/77608.html}{ISO/IEC}, \href{https://standards.ieee.org/initiatives/autonomous-intelligence-systems/}{IEEE}, and the U.S. \href{https://nvlpubs.nist.gov/nistpubs/ai/NIST.AI.100-1.pdf}{NIST} provide additional guidance.
\item These initiatives encourage the responsible and human-centric use of AI, focusing on principles like privacy, data governance, accountability, and human oversight.
\end{itemize}

The legislative overhead (globally - taken in aggregate) is very high, and there's growing concern about the energy and carbon footprint of the technology \cite{wu2022sustainable}. 


\subsubsection{US's Sectoral Approach to AI Regulation}
\begin{itemize}
\item US AI governance is dispersed across various federal agencies and tailored to specific sectors.
\item The Federal Trade Commission (FTC), wielding its \href{https://www.ftc.gov/business-guidance/blog/2021/04/aiming-truth-fairness-equity-your-companys-use-ai}{authority}, is actively involved in AI regulation. Its commitment to enforcing fair AI use was demonstrated by opening an \href{https://www.washingtonpost.com/documents/67a7081c-c770-4f05-a39e-9d02117e50e8.pdf?itid=lk_inline_manual_4}{investigation} into OpenAI's chatbot ChatGPT.
\item The Equal Employment Opportunity Commission (\href{https://www.eeoc.gov/newsroom/eeoc-releases-new-resource-artificial-intelligence-and-title-vii}{EEOC}) and the Consumer Financial Protection Bureau (\href{https://www.consumerfinance.gov/about-us/blog/algorithms-artificial-intelligence-fairness-in-home-appraisals/{CFPB}) are other examples of active sectoral regulators for AI.
\item States are also showing interest in AI regulation, with California introducing \href{https://leginfo.legislature.ca.gov/faces/billTextClient.xhtml?bill_id=202320240AB331}{AB 331}, a law specifically targeting automated decision tools.
\item Public discourse suggests potential for a broader approach, incorporating AI requirements in a comprehensive national privacy law, like the proposed \href{https://www.commerce.senate.gov/services/files/9BA7EF5C-7554-4DF2-AD05-AD940E2B3E50}{American Data Privacy and Protection Act}.
\item In addition to actively governing algorithms, \href{https://carnegieendowment.org/2023/07/10/china-s-ai-regulations-and-how-they-get-made-pub-90117}{China recently introduced AI regulations} targeting generative AI and fake news.
\end{itemize}
The FTC has published a \href{}{blogpost} discussing the legal implications of AI-generated deception under the FTC Act. As synthetic media becomes more widespread, understanding the legal landscape is crucial for businesses involved in creating, distributing, or using AI-generated content. The FTC Act governs deceptive or unfair practices, including synthetic media and generative AI tools. Businesses should consider liability assessment, risk mitigation, deterrence measures, avoiding misrepresentation and false advertising, and post-release detection and monitoring. Other legal frameworks, such as copyright and trademark laws, defamation, and privacy rights, may also apply. The FTC emphasizes the importance of considering the broader social and ethical implications of these technologies and calls for collaboration among legal professionals, regulators, and industry stakeholders to ensure responsible development and use of AI-generated content. It feels like even this comparatively swift response is too little too late. 

\subsubsection{EU's Comprehensive AI Regulatory Approach}
\begin{itemize}
\item The European Commission (EC) introduced the \href{https://digital-strategy.ec.europa.eu/en/policies/regulatory-framework-ai}{draft AI Act in April 2021}, aiming to be the EU's first comprehensive, cross-sectorial regulation focusing on AI.
\item The Act will categorize AI systems based on risk, impose fines for non-compliance, and is currently in the negotiation phase.
\item The \href{https://commission.europa.eu/business-economy-euro/doing-business-eu/contract-rules/digital-contracts/liability-rules-artificial-intelligence_en}{AI Liability Directive} and a revision of sectoral safety legislation, including for \href{https://law.stanford.edu/publications/machine-learning-eu-data-sharing-practices/}{machinery and general product safety}, are also part of the EU's AI strategy.
\end{itemize}

The EU is first mover on this, and they have over-corrected for their lack of knowledge (arguably fair enough):\
The EU regulation has been passed on 14/6 and classifies AI systems into four risk categories: unacceptable risk, high risk, limited risk, and minimal risk. Unacceptable risk AI systems will be prohibited, while high-risk AI systems will be subject to strict requirements. Any training of a model is automatically a foundational model (annoyingly) and therefore high risk. Getting a compliant model will require a demonstration of deep understanding of the workings of the model. It's unclear how anyone will accomplish this and it may end up being a defacto ban on trained models and possibly even optimised ones (\hyperref[sec:LoRA]{LoRA}). Any product derived from a \textbf{compliant} foundational model will be deemed acceptable by default. This question of compliant foundation models is absolutely key as we plan through the 3 year grace period which the EU has allowed. Short of a proper external legal assessment we \textit{must} assume that Immersive is in scope in terms of it's projects, because of the global reach of the law. Any business doing any business in the EU is exposed. Stanford University Centre for Research on Foundation Models have done their own assessment on the compliance of the current models, and they simply aren't \ref{fig:euAIcompliance}. Bloom from Huggingface is closest and is `perhaps' \href{https://huggingface.co/BelleGroup/BELLE_BLOOM_GPTQ_4BIT}{usable in optimised modes} on cloud \href{https://lambdalabs.com/nvidia-h100-gpus}{hardware} \cite{dettmers2022case}. I suggest we just plough on with whatever is most performant but keep and eye on it.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{euaicompliance}
    \caption{Stanford's assessment of the compliance of current foundation models vs the EU AI act.}
    \label{fig:euAIcompliance}
\end{figure}

Some other things can be high risk too, like external HR software. Limited-risk and minimal-risk AI systems will be subject to less stringent requirements. 
\begin{itemize}
  \item \textbf{Safety and Transparency:} AI systems used within the EU must be safe, transparent, traceable, non-discriminatory, and environmentally friendly. These systems should be overseen by humans to prevent harmful outcomes.
  \item \textbf{Risk-Based Categories:} The EU AI Act categorizes AI systems based on risk levels, which include unacceptable risk, high risk, limited risk, and a separate category for generative AI like ChatGPT.
  \item \textbf{Banned Practices:} Certain practices, like live facial recognition and scraping of biometric data from social media, are prohibited.
  \item \textbf{Transparency for Generative AI:} Companies may have to publish summaries of copyrighted material used for training their systems, which could be problematic for LLMs due to the vast amount of data involved in training.
  \item \textbf{Designing Prohibitions for Illegal Content:} AI systems should be designed to prevent the generation of illegal content.
  \item \textbf{AI-Generated Content Disclosure:} People must be informed when they are interacting with AI-generated content.
  \item \textbf{High-Risk Activities:} High-risk activities, such as certain uses of AI in law enforcement, will be subjected to tighter regulation.
  \item \textbf{Pre-Deployment Risk Assessments:} The EU proposes to implement a pre-deployment risk assessment process for high-risk models before they are released to the public.
  \item \textbf{Open Source Carve-out:} The act includes provisions for open source AI, but there are exclusions for large open source "Foundation Models" like GPT.
  \item \textbf{Training Data Documentation:} Companies may need to comprehensively document and be transparent about the copyrighted material used in the training of their algorithms, which could be challenging due to the amount and diversity of training data used.
\end{itemize}

It is somewhat unclear where these delimiters are; they will have to clarify it at some point. Burges Salmon Solicitors have provided a public access flowchart which is pretty helpful and is in Figure \ref{fig:euaiflowchart}.

\ref{fig:EUAIflowchart.pdf}. 
\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{euaiflowchart.pdf}
    \caption{EU AI legislation.}
    \label{fig:euaiflowchart}
\end{figure}


The USA and UK meanwhile will likely use the court system to iteratively establish these boundaries over time, though there will clearly be guidance soon(ish). Nobody wants to get caught up in courts around AI.

There will be legislative focus on human oversight. The regulation will require that all AI systems have human oversight, meaning that humans will be able to understand and control how the AI systems operate. This is intended to help ensure that AI systems are used in a safe and ethical manner. I think this is fine in the context of physical events in that we can simply record the current session to text, and discard afterwards, allowing users to ``come to the information desk'' and discuss their signed waiver. \par 

The regulation will require that AI systems be transparent, meaning that users will be able to understand how the AI systems work and how they make decisions. Again, this just goes in the waiver. I am hopeful that there will be boilerplate terms we can use for each jurisdiction in the context of deployed AI. The regulation will require that AI systems be accountable, meaning that the developers and users of AI systems will be responsible for the consequences of their use. This is less clear to me, because we will at `least' be users, so we might need a bit of advice on the implications here.\par
The draft AI regulation intersects with GDPR in a number of ways. For example, GDPR requires that personal data be processed in a fair and transparent manner. So again, it will require that AI systems that process personal data be transparent and accountable. Additionally, the GDPR prohibits the processing of personal data for certain purposes, such as profiling. It rightly prohibits the use of AI systems for social scoring. Non of that is a problem if we don't collect ANY user data extrinsic to the session when we deploy to the public.\par
The regulation will apply to all AI systems that are developed, placed on the market, or \textbf{used in the European Union}, and we can expect that many countries will simply copy/paste this legal framework. It will be enforced by national authorities in each EU member state, which is suggestive of a degree of (risky) legislative arbitrage potential. Perhaps most annoyingly at a pragmatic level, there are a number of technical requirements for AI systems, such as accuracy, and fairness. I suspect we can explain to users that the technology is nascent and use a high quality model to demonstrate best effort, training and testing against our local event dataset. All regulation will also include a number of procedural requirements, such as requirements for risk assessment and documentation. The penalties in the EU for violating the regulations will be significant. For example, up to 4\% of \textbf{global} annual turnover. The timeline for the adoption of the laws is still being negotiated, though the European Commission has stated that it expects the end of 2023, crucially with a two year phase in. This still means pretty much means `anything we do', since there is an extrinsic capture clause in EU law for international companies selling at all into the EU. This is the legislation to watch basically.\par
The Online Safety Bill is the most relevant UK legislative proposal pertaining to AI, as it includes a number of provisions that specifically address the use of AI by online platforms. The bill requires \textit{online} platforms to take steps to prevent the spread of harmful content, \textbf{including content that is generated by AI systems}. The bill also requires online platforms to be more transparent about how they use AI systems and to give users more control over how their data is used. The penalties for non-compliance with the legal provisions in the UK vary depend on the law that is being breached. Fines of up to £10 million for breaches of the DPA 2018. The information commissioners office has \href{https://ico.org.uk/for-organisations/uk-gdpr-guidance-and-resources/artificial-intelligence/guidance-on-ai-and-data-protection/how-should-we-assess-security-and-data-minimisation-in-ai/}{issued vague guidance} and can enforce through notices requiring companies to take steps to comply with the law. The UK seems less burdensome at this time, \textbf{but a quirk of the law gives \href{https://webdevlaw.uk/2022/11/21/a-quick-hypothetical-situation-or-your-crash-introduction-to-the-real-world/}{genuine legal peril} for C-Suite individuals}. I have been quoted nearly £600/hr \href{https://www.linkedin.com/in/barry-scannell-bbb5aa207/}{by this LinkedIn guy}, for legal and risk assessment in the UK.\par
Sunak has signalled that his government wishes the UK to be regarded as a global leader in AI safety. This will obviously engender both opportunities and risks. The new lead of the UK foundation model taskforce, Ian Hogarth, has been quite vocal over the last few years on these matters, and seems a knowledgeable and well considered appointment.\par
In 2018, Hogarth's key concern around AI was the implications of the potential acceleration of AI development and deployment, which he referred to as ``AI nationalism''. He argued that nations would enter into a competitive race to advance AI technology, triggering geopolitical tension and even conflict. He also mentioned the risk of nations stockpiling AI technology and preventing others from accessing it (something we can see in the USA CHIP act), and noted the need for an international, cooperative approach to managing AI.\par
In 2021, Hogarth’s perspective evolved to a more focused concern about the swift progress of AI development, especially in the realm of Artificial General Intelligence (AGI), which he refers to as ``Godlike AI''. This shift was based on his experiences and conversations within the tech industry. He raised the alarm about the rapid speed at which private companies are advancing towards AGI without proper oversight and regulation.  He expressed concern that the race to develop AGI was taking place in a small community of tech companies, without democratic involvement or consideration of potential risks to the human race. These are valid concerns.\par
He, like I, thinks there has been an increasing rush towards the development of AGI, and the people involved seemed more focused on the potential benefits rather than considering the risks. \par 
Despite this, he remains fundamentally optimistic about the potential of science and technology to transform our lives for the better, provided it is done safely. He will have a direct role in shaping the future of AI regulation in the UK. His recognition of the need for governments to get more involved, and for more people to have a say in the AI conversation, potentially represents an invitation and opportunity for businesses. 

\subsubsection{UK Legal Position}

\begin{itemize}
    \item \textbf{Source Reference:}
    \begin{itemize}
        \item This summary is based on the "Responsible and Trustworthy AI" report published by the UK. The full report can be accessed \href{https://iuk.ktn-uk.org/wp-content/uploads/2023/10/responsible-trustworthy-ai-report.pdf}{here}.
    \end{itemize}

    \item \textbf{Strategic Objective:}
    \begin{itemize}
        \item The UK Science and Technology Framework (March 2023) identifies AI as one of five critical technologies. The UK is seeking to build a strategic and globally competitive advantage in AI to become a science and technology superpower by 2030.
    \end{itemize}

    \item \textbf{Core Principles of Responsible and Trustworthy AI (RTAI):}
    \begin{itemize}
        \item \textit{Transparency and Explainability}: Essential for understanding AI systems.
        \item \textit{Safety, Security, and Robustness}: Ensuring AI systems are robust, safe, and secure.
        \item \textit{Non-maleficence}: AI must not harm individuals, society, or the environment.
        \item \textit{Privacy}: Protecting personal information and addressing surveillance concerns.
        \item \textit{Fairness and Justice}: Promoting equality and addressing biases.
        \item \textit{Accountability}: Organisations must take ownership of AI actions and decisions.
    \end{itemize}

    \item \textbf{Policy Direction and Legislation:}
    \begin{itemize}
        \item Guiding the development, deployment, and use of RTAI across the AI lifecycle.
        \item Seeking international consensus on RTAI principles for global alignment.
    \end{itemize}

    \item \textbf{Challenges and Implementation:}
    \begin{itemize}
        \item AI's transformative impacts pose challenges in responsible application.
        \item Necessity for trade-offs when RTAI principles conflict.
        \item Notable cases of principle violations, such as government predictive algorithms and Clearview AI Inc. scandal.
    \end{itemize}

    \item \textbf{Stakeholder Responsibilities:}
    \begin{itemize}
        \item Developers and industry representatives.
        \item Government bodies, regulators, and policymakers.
        \item Standards bodies for technical standards.
        \item Funders and investors supporting RTAI development.
        \item Users, customers, and researchers in public debate.
        \item Advisory bodies and social actors shaping public debate.
    \end{itemize}

    \item \textbf{Guidance and Tools:}
    \begin{itemize}
        \item Existence of guidance documents and tools for implementing RTAI.
        \item Need for more granular operationalisation techniques due to voluntary and variable quality of these tools.
    \end{itemize}
\end{itemize}


\subsection{Humans and AI, horizon scanning}
As AI becomes increasingly integrated into various aspects of our lives, it is poised to transition from being a mere tool to becoming an integral companion and collaborator. The potential trajectory of this evolution covers a wide range of areas, including equity, environment, education, health, governance, and more.
\begin{figure}[ht]
\centering
\includegraphics[width=0.19\textwidth]{base_output_00002_.png}
\hfill
\includegraphics[width=0.19\textwidth]{base_output_00003_.png}
\hfill
\includegraphics[width=0.19\textwidth]{base_output_00005_.png}
\hfill
\includegraphics[width=0.19\textwidth]{base_output_00006_.png}
\hfill
\includegraphics[width=0.19\textwidth]{base_output_00007_.png}
\caption{A progression of human-AI interaction, oneshot collaboration between ChatGPT and SDXL. Placeholder.}
\end{figure}

\subsubsection{The Evolution of Human-AI Interaction: Soon, Next, and Later}
This journey of human-AI integration can be broadly divided into three phases: 'Soon', 'Next', and 'Later'. Each phase brings unique challenges and opportunities.\par 

\textbf{The 'SOON' phase} focuses on Digital Literacy, Data Privacy, and Algorithmic Bias. It's critical that individuals understand how to use AI and digital technologies to access information and services. Additionally, as AI systems often rely on personal data, ensuring privacy and mitigating biases embedded in AI algorithms are key challenges. \par

\textbf{The 'NEXT' phase} will see the rise of Biome AI, AI Ethics \& Safeguarding, and Ambient Education. In this phase, AI will become more integrated into our biological lives and our everyday environments. It will be imperative to ensure the responsible use of AI as its influence grows. This phase will require a focus on developing robust ethical frameworks for AI use, and creating ambient educational environments where learning is facilitated by AI.\par 

\textbf{The 'LATER' phase} anticipates the emergence of Fully Autonomous Systems, where AI will become so advanced and reliable that it can operate without human supervision in various sectors, leading to unprecedented levels of productivity and efficiency. Another exciting aspect of this phase is the intersection of AI and Mental Health. AI companions will be capable of understanding human emotions and mental states, providing psychological support and therapeutic interventions. They could assist in managing mental health conditions and improving overall well-being.

\subsection{Human flourishing and expression}
\paragraph{Celebrating Human Diversity: Now to Later}\par
As AI becomes more integrated into our daily lives, it will play a crucial role in celebrating and promoting human diversity. AI systems will be designed to understand, respect, and adapt to a wide range of human experiences, perspectives, and identities. They will help us to better understand ourselves and each other, breaking down barriers and fostering a more inclusive society. Furthermore, by acknowledging the unique forms of intelligence exhibited by AI, we can redefine what intelligence means in a diverse society.
\paragraph{AI supported creativity: Soon to Next}\par
In the future, we also foresee the rise of AI and Creativity, where AI will not only assist in creating art, music, and literature, but will also be capable of original creative thought, leading to a renaissance of AI-generated creativity that will reshape our cultural landscape. Another exciting prospect is the development of Diverse AI. Just as human diversity is celebrated, AI will be designed with diverse "personalities" and ways of thinking, leading to a richer and more nuanced interaction between humans and AI.

\paragraph{Equity: Now to Next}\par
By democratizing resources, and lowering the marginal cost of education to zero globally, AI will play a pivotal role in reducing socio-economic disparities. However, it's crucial to ensure that AI advancements are distributed equitably and don't reinforce existing social inequities.
\paragraph{Secret Learnings for Children: Next to Later} \par
AI education will include playful, memorable, and slightly subversive learning experiences. AI educators will foster independence and trust in children by providing private, magical moments of learning. Some of these moments might occur in secret, away from adult supervision, encouraging children to explore, experiment, and learn in their own unique ways. All children should have the opportunity to grow up with headphones that contain a local AI informational agent, even without connection to the internet. Access of opportunity increases.
\paragraph{The age of the productive tinker: Later}\par
Increasingly a simple set of small specialised chips (ASICs) will allow low power inference using AI. This will produce an explosion of gadgets for niche applications. As an example AI will revolutionize the fashion industry by co-designing 3D printed single-use clothing tailored to individual preferences. These clothes could be made from environmentally friendly materials, suitable for recycling after use.
\subsubsection{Environment}
The manifestation of AI as a tool to support and celebrate human diversity also has profound implications for our interaction with the environment. As AI systems become more attuned to understanding and adapting to a wide range of human experiences and perspectives, they also have the potential to significantly enhance our relationship with the natural world. This transition from human flourishing to a more sustainable interaction with our environment is the next critical stage in our evolving relationship with AI.
\paragraph{Resilience and collaborative management} 
AI's role in predicting and monitoring environmental changes, optimizing resource consumption, and enhancing waste management will become widespread, while the carbon footprint of AI technologies will need to be minimized. Additionally, future scenarios include AI's role in Climate Change and Wildlife Conservation. Advanced AI models will help in predicting and mitigating the effects of climate change, assisting in the planning and execution of climate resilience strategies at local and global levels. AI will also play a critical role in wildlife conservation, from monitoring endangered species and their habitats, to predicting and preventing potential threats. 

\paragraph{Supporting our place: Later}: 
AI will support human relationships with nature by monitoring and managing our physical health at a micro-level. These systems will provide educational information about our natural environment, helping us make more sustainable choices.
\subsection{Holistic health}
Our interaction with the environment is intrinsically linked to our overall health and well-being. AI’s role in environmental management can directly impact our personal health. As AI technologies evolve to help us predict and respond to environmental changes, optimize resource consumption, and enhance waste management, they also pave the way for more holistic approaches to health management. This progression from environmental stewardship to personalized health care is the next evolution in the integration of AI into our daily lives.
\paragraph{Personal Health Management: Now to Next}: 
AI will also support our relationships with our own health and internal biome. Personalized AI systems will analyze and respond to changes in our biomes to optimize our health, making recommendations based on our specific needs and preferences.
\paragraph{Lifetime Support Structures: Now to Later}
AI will serve as a form of lifetime support, offering guidance throughout various stages of life. These AI systems will learn patterns, habits, and preferences over time, providing customized assistance, reminders, and suggestions to improve wellbeing and productivity.
\subsection{The age of the informational Agent}
As trust in the internet evolves, the situation will change and adapt as people learn to use informational agents. Intentional UX will allow users to ask their AI to bring them the information they want from a far more decentralized and confusing internet. This will promote incredible diversity in humans as they fracture somewhat into informational enclaves.

Two future scenarios include the rise of AI in Truth Verification and Education. AI will become sophisticated enough to verify the truthfulness of information on the internet, combating the spread of misinformation and ensuring that users have access to accurate and reliable information. AI will also become an integral part of education, acting as a personalized tutor that adapts to each student's learning style and pace, revolutionizing the way we learn and acquire new skills.

\paragraph{Money will change: Next -Later}: Money will increasingly be spent by machines on behalf of human intent. Algorithms will bargain and arbitrage on behalf of their owner/user, for human and machine services, and for ideas, alorithms, and good; gloablly. This will smooth out the operation of money globally.

\paragraph{Ubiquitous multi-modal UX: Next to Later}
The future will see the rise of ubiquitous displays, computing \cite{lyytinen2002ubiquitous}, and interfaces - screens and projections seamlessly integrated into our environments. These displays will not only provide information and entertainment but will serve as interfaces for our interactions with AI. Gesture may come to the fore, and subvocalisation to talk to personal AIs will be possible.


\subsection{Risks, Responsibilities and Mitigation Strategies for AI in Events}

\subsubsection{Risks and Responsibilities}

\begin{itemize}
\item \textbf{Privacy and data protection} - The AI system will likely process significant personal data, so complying with regulations like GDPR is crucial. Strategies like data minimization, transparency, and consent mechanisms should be implemented.

\item \textbf{Algorithmic bias} - With hyper-personalization, there is a risk of discriminatory outcomes if the algorithms embed societal biases. Rigorous testing for fairness and regular audits are needed.

\item \textbf{Transparency} - The EU AI Act requires high levels of transparency for users. The company must ensure the AI logic is explainable and accessible.

\item \textbf{Cybersecurity} - Customer data could be vulnerable, so strong cybersecurity protections are vital, like encryption and access controls.

\item \textbf{AI safety} - Irresponsible AI could recommend harmful events. Oversight systems like human-in-the-loop review are important safeguards.

\item \textbf{Legal liability} - If AI-recommended events cause harm, legal liability questions arise. The company should clarify liability through contracts and insurance.

\item \textbf{Copyright} - Training datasets likely contain copyrighted content. Proper licensing and credits are needed.

\item \textbf{Environmental impact} - Energy usage and carbon footprint of large AI models should be managed through efficiency measures.

\item \textbf{Industry disruption} - Jobs like event planners could be impacted. Transition support for affected workers can demonstrate social responsibility.
\end{itemize}

\subsubsection{Mitigation Strategies}

\begin{itemize}
\item Perform comprehensive risk assessments accounting for EU regulations.

\item Implement "ethics by design" in development and deployment.

\item Establish oversight boards, audits, and impact assessments.

\item Clearly communicate AI capabilities, limitations and roles to users.

\item Develop strict protocols for obtaining user consent. Enable user controls over data.

\item Test extensively for algorithmic bias and other harms using diverse datasets.

\item Engineer transparency into the AI models and provide explanations of outputs.

\item Implement cybersecurity best practices and controls like multi-factor authentication.

\item Establish human oversight procedures and feedback loops to check AI recommendations.

\item Clarify legal culpability and seek appropriate insurance coverage.

\item Formally credit all copyrighted training data. Seek explicit licensing where feasible.

\item Adopt energy-efficient computing infrastructure. Purchase carbon offsets.

\item Provide job retraining opportunities to affected professionals.
\end{itemize}



==> 09_ethics_law.tex <==
\subsection{Ethics \& Impact}
AI ethics is now a hot topic even outside of the academic fields which have previously wrestled with these issues. These new systems are thought likely to be able to impact all human activity \cite{eloundou2023gpts}. \par
The Centre for Humane Technology \href{https://www.humanetech.com/key-issues}{highlight the negative assessment} of the risk of Large Language Models, stating that major advancements in AI are coming and society needs to address the issues before they become `entangled'. The misalignment problem with social media has not been fixed, and this is where Harris and Raskin made their name. Their focus is not on AGI apocalypse scenarios but rather on the potential consequences of rapid AI advancements. AI has evolved significantly since 2017. They somewhat hyperbolically call such models `golems', in reference to their emergent capabilities. They would like society to address the potential risks of LLMs before they become entangled in society and to better understand and manage their impact.\par
They highlight author \cite{harari2014sapiens} Harari's quote: \textit{``What nukes are to the physical world, AI is to the virtual and symbolic world.''} - and this quote feels very compelling when held up against our assertions about cryptographic end points and trust.\par
Rosenburg describes \href{https://bigthink.com/the-present/danger-conversational-ai/}{`The AI manipulation problem'} which refers to the emerging risk of real-time engagement between a user and an AI system that can impart targeted influence, sense the user's reactions, and adjust tactics to maximize persuasive impact. This can occur through natural spoken interactions with photo realistic virtual spokespeople that look, move, and express like real people. Conversational AI can push individual emotional buttons by adapting to personal data and analyzing real-time emotional reactions, becoming more skilled at playing each user over time. This presents a serious concern as it can be used to influence individuals and broad populations in ways that may be damaging to society \cite{Rosenberg2023}. \par
As AI models improve, they are generating their own data for reinforcement learning, with humans only needed to train the reward function. The advancements are not limited to algorithms and APIs; even hardware is advancing rapidly due to AI, as shown by Nvidia's research on using AI to improve chip design.\par
GPT-4 is breaking its \href{https://nanothoughts.substack.com/p/reflecting-on-reflexion}{own records} through self-reflection. This reflection paper has caught global attention and shows GPT-4's ability to improve upon its mistakes, and enhance its performance in a variety of tasks \cite{shinn2023reflexion}. The process of self-reflection has been observed in other research papers as well, demonstrating its effectiveness in improving model outputs.\par
The ground breaking Huggingface GPT model can draw upon thousands of other AI models to perform tasks involving text, image, video, and question answering \cite{shen2023hugginggpt}. The Hugging GPT paper reveals a model that can connect numerous AI models for solving complex tasks, using language as an interface. It can perform tasks such as describing and counting objects in a picture, generating images and videos, deciphering invoices, and even describing them in perfectly simulated human voices.\par
The rapid advancements in AI are causing commercial pressure, pushing companies like Google to catch up with the likes of OpenAI. With self-improvement, tool use, hardware advances, and commercial pressure, the future of AI seems to be on a trajectory of rapid growth and development. The most recent comparator is the emergence of the iPhone and death of Adobe Flash \cite{horton2019death}, but this is orders of magnitude beyond that and likely most analogous to the industrial revolution \cite{trajtenberg2018ai}. \par 
\href{https://www.key4biz.it/wp-content/uploads/2023/03/Global-Economics-Analyst_-The-Potentially-Large-Effects-of-Artificial-Intelligence-on-Economic-Growth-Briggs_Kodnani.pdf}{A Goldman report} sees 25\% of roles basically wiped out. Even OpenAI themselves published similar findings \cite{eloundou2023gpts}. The systems can already pass almost all human examinations with ease, causing immediate existential harm to education assessment systems.\par 
The risks of generative AI are well covered by a \href{https://www.citizen.org/article/sorry-in-advance-generative-ai-artificial-intellligence-chatgpt-report/}{Public Citizen article}, and are simply listed below to get us started. It is a huge and well researched report and this list doesn't do it justice:
\begin{itemize}
\item A sharp increase in political disinformation;
\item Intensified, widespread consumer and financial fraud;
\item Intrusive privacy violations beyond those already normalized by Big Tech;
\item Harmful health impacts, from promotion of quack remedies to therapeutic malpractice;
\item Amplification of racist ideas and campaigns;
\item Destruction of livelihoods for creators;
\item Serious environmental harm stemming from generative A.I.’s intense energy usage;
\item The stripping of the information commons;
\item Subversion of the open internet;
\item Concentration of economic, political, and cultural power among the tiny number of giant companies with the resources to develop and deploy generative A.I. tools.
\end{itemize}

Research suggests that LLM outputs cannot be discriminated from human output in meaningful ways, casting shade across all assessed measures of humans in written form \cite{sadasivan2023can} from this point forward. Michal Zalewski \href{https://lcamtuf.substack.com/p/llms-a-bleak-future-ahead}{says}: \textit{``Instead of taking sides in that debate, I’d like to make a simpler prediction about LLMs as they operate today. It is possible that barring urgent intervention, within two decades, most of interactions on the internet will be fake. It might seem like an oddly specific claim, but there are powerful incentives to use LLMs to generate inauthentic content on an unprecedented scale — and there are no technical defenses in sight. Further, one of the most plausible beneficial uses of LLMs might have the side effect of discouraging the creation of new organic content on the internet.''}
Within generative machine learning there has been a raging debate between `some' of the artists whose original works were `scraped' into the \href{https://laion.ai/}{LAION} open dataset. There are numerous legal battles under way around copyright and disclosure of information. This disclosure is itself written into the EU AI bill, and will favour incumbents who have enough scale to retrofit an analysis. Adobe claim their Firefly product is built upon their own dataset but clearly contains wider examples of artists styles. Reddit, and open source programmers on GitHub are looking to sue based on the the large language scrapes. It's too early to say how this might go.\par
AI safety and the challenges associated with managing an AI system's output are important considerations. Efforts have been made to ensure AI safety over the years, but the pace of change may be outstripping the ability of the industry and researcher to keep up. Finding the right balance between allowing users to express themselves and drawing the line on harmful or offensive content is a difficult task. Defining concepts like hate speech and harmful output, as well as aligning AI systems with human values and preferences, are complex challenges. Ideally, a democratic process would involve people from different perspectives coming together to decide on rules and boundaries for AI systems. However, implementing such a process is not straightforward, and developers must remain heavily involved in decision-making while still seeking input from a broader audience.\par
It is beyond the scope of this text to dig far into these issues, but they have serious implications for anyone working in the space. \par 
\subsubsection{AI's lying heart}
Large language model systems, at this time, are given to making things up. They `hallucinate' very cogently \cite{azamfirei2023large}, presenting completely erroneous assertions and data as facts, with \href{https://news.artnet.com/art-world/chatgpt-art-theory-hal-foster-2263711}{figures to back them up}. Perhaps counter intuitively this problem extends into pure mathematical realms, with seemingly simple arithmetic causing the systems problems. Both of these are the same problem, the models descend the most statically plausible path toward an output based pretty much on the last character generated along the vector into the n dimensional algebra space. This is being ameliorated through self checking \cite{manakul2023selfcheckgpt}, human reinforcement learning \cite{ouyang2022training}, and integration of specialised tools \href{https://writings.stephenwolfram.com/2023/01/wolframalpha-as-the-way-to-bring-computational-knowledge-superpowers-to-chatgpt/}{like Wolfram Alpha}, behind the models.\par 
Media outlets such as The Guardian are rushing to publish open guidelines on \href{https://www.theguardian.com/commentisfree/2023/apr/06/ai-chatgpt-guardian-technology-risks-fake-article?}{how they intend to deal} with the problem of GPT based article research, and it seems that \href{https://www.bbc.co.uk/news/technology-65202597}{legal challenges} will quickly mount up. With that said, the UK government is currently signalling a \href{https://www.gov.uk/government/publications/ai-regulation-a-pro-innovation-approach}{``pro-innovation''}, hands off approach to AI, and is \href{https://www.gov.uk/government/news/initial-100-million-for-expert-taskforce-to-help-uk-build-and-adopt-next-generation-of-safe-ai}{investing significantly} in supporting the technology.
\subsubsection{Alignment and take-off of AGI}
AI has the potential to significantly improve quality of life, but it is essential to ensure that it remains aligned with human values and does not harm or limit humanity. Alignment in language models trys to address this by incorporating strategies, which can be broadly categorized into the following areas:
\begin{itemize}
\item \textbf{Pre-training} In the initial stage, models are trained on a large dataset containing diverse text from the internet. This allows them to learn grammar, facts, reasoning abilities, and some level of world knowledge. However, they can also learn biases present in the data. Alignment efforts at this stage may involve dataset choices, monitoring, and some feedback to reduce reduce obvious biases.
\item \textbf{Fine-tuning} After pre-training, models are fine-tuned on a narrower, more specific dataset, often with human-generated examples and labels. During fine-tuning, alignment efforts can include generating clearer instructions for human reviewers, providing them with guidelines and feedback, and iteratively refining the process to improve the model's behaviour. Things like ranked lists of responses from the system would go in this stage. This is the ``human reinforcement learning'' which has so invigorated LLMs recently \cite{perez2022discovering}.
\item \textbf{Evaluation} Assessing the performance and safety of a language model is crucial for alignment. This can involve creating evaluation metrics, benchmarks, and tests to measure the model's progress in terms of safety, usefulness, and alignment with human values. Some of these are encoded inline with the model generation and are called `hyperparameters'. Two important hyperparameters that influence the generated text are frequency penalty and presence penalty. Frequency penalty affects the repetition of tokens in the generated text by modulating the probability distribution of tokens. A positive frequency penalty value discourages the model from choosing frequently occurring tokens, leading to a more diverse and sophisticated vocabulary. Presence penalty influences the generation of tokens that have already appeared in the generated text. A higher presence penalty value discourages the model from repeating tokens or phrases, ensuring a more cohesive and engaging output. On the other hand, a lower presence penalty value allows the model to generate text with repeated tokens or phrases, which can lead to redundancy and reduce the overall coherence of the text.\par 
So called use of `Red Teams' goes in this section, but much of this has recently been done live on alpha and beta public testing. 
\item \textbf{Safety mitigations} Addressing risks associated with harmful outputs, non-consensual content, and other safety concerns is an essential aspect of alignment. Techniques like more reinforcement learning from human feedback, rule-based filters, and output constraints can be employed to reduce harmful outputs and improve model safety. These feedback loops at the end of the process carry a disproportionate weight in the models, and it is at this stage that the most noticeable change is sometimes introduced. It is critical to get the maximum global public engagement during this final feedback into the system, from policy-makers and diverse human response feedback. It's not clear this is yet happening. Even Altman, the CEO of OpenAI admits that the models likely reflect the training choices of San Francisco `Tech Bros' in this moment. That is clearly not good enough.
\end{itemize}
Altman, says they have optimised their approach based on aiming for earlier AGI, but a slow AGI ``takeoff'', ie, the dfference between a gradual understandable creep toward a general intelligence, vs ``AI FOOM'' \cite{yudkowsky2008hanson}. They have a weighted risk matrix, but no clear ideal -yet- as to what the tools look like to keep the AGI "aligned" with humanity. Starting fast, but asserting slow and steady about the emergent behaviour part seems optimistic at best. Nonetheless this is likely the best/only approach, assuming it' possible. The only alternative is literally the ``Butlerian Jihad'' from Herberts' Sci-Fi DUNE.\cite{song2018preventing}.\par
There is a possibility that AI could become misaligned as it gains superintelligence, and it is essential to acknowledge and address this risk. 
AI technology, such as GPT-4, has shown exponential improvement, raising concerns about AI takeoff, which could happen rapidly within days. While GPT-4's performance has not been surprising to some, its impact highlights the need to increase technical alignment work and continually update the understanding of AI safety.\par
It's noteworthy that industry luminaries such as Yoshua Bengio, Turing Prize winner, Stuart Russell, director of the Center for Intelligent Systems, Elon Musk, and Steve Wozniak, Co-founder of Apple co-signed an \href{https://futureoflife.org/open-letter/pause-giant-ai-experiments/}{open letter} requesting a 6 month pause on the development of these systems. For what it's worth the author also signed. The narrative needs time to catch up. To be clear it won't happen, but the signalling here is part of building the awareness that is sorely lacking. 
\subsubsection{Industry capture, and failure to democratise}
Financial time article, integrate:
\begin{tcolorbox}[enhanced, frame style={fill=lightgray}, interior style={fill=lightgray}]``There's a colossal shift going on in artificial intelligence - but it's not the one some may think. While advanced language-generating systems and chatbots have dominated news headlines, private AI companies have quietly entrenched their power. Recent developments mean that a handful of individuals and corporations now control much of the resources and knowledge in the sector - and will ultimately shape its impact on our collective future. The phenomenon, which AI experts refer to as "industrial capture", was quantified in a paper published by researchers from the Massachusetts Institute of Technology in the journal Science earlier this month, calling on policymakers to pay closer attention. Its data is increasingly crucial. Generative AI - the technology underlying the likes of ChatGPT - is being embedded into software used by billions of people, such as Microsoft Office, Google Docs and Gmail. And businesses from law firms to the media and educational institutions are being upended by its introduction.
The MIT research found that almost 70 per cent of AI PhDs went to work for companies in 2020, compared to 21 per cent in 2004. Similarly, there was an eightfold increase in faculty being hired into AI companies since 2006, far faster than the overall increase in computer science research faculty. "Many of the researchers we spoke to had abandoned certain research trajectories because they feel they cannot compete with industry - they simply don't have the compute or the engineering talent," said Nur Ahmed, author of the Science paper. In particular, he said that academics were unable to build large language models like GPT-4, a type of AI software that generates plausible and detailed text by predicting the next word in a sentence with high accuracy. The technique requires enormous amounts of data and computing power that primarily only large technology companies like Google, Microsoft and Amazon have access to. Ahmed found that companies' share of the biggest AI models has gone from 11 per cent in 2010 to 96 per cent in 2021. A lack of access means researchers cannot replicate the models built in corporate labs, and can therefore neither probe nor audit them for potential harms and biases very easily. The paper's data also showed a significant disparity between public and private investment into Al technology. In 2021, non-defence US government agencies allocated \$1.5bn to AI. The European Commission planned to spend \$1.5bn. Meanwhile, the private sector invested more than \$340bn on Al in 2021.''
\end{tcolorbox}
\subsubsection{Cybersecurity implications}
It seems clear to all observers of the potential LLMs to be leveraged in supranational misinformation campaigns, zero-day exploits, and other geopolitical threats. It's appropriate to contextualise American export restrictions on powerful GPU and TPU hardware to China and Iran, and the implications of LLMs being "in the wild" and easily retrained for nefarious purposes. These powerful tools can be weaponised by malicious actors to create a new frontier of cybersecurity threats. 
\begin{itemize}
\item Supranational Misinformation Campaigns: 
LLMs can be easily retrained and used to generate convincing disinformation, thereby escalating the effectiveness of misinformation campaigns. As LLMs become more accessible, nation-states and non-state actors can utilise these technologies to create more targeted, sophisticated, and persuasive disinformation. This could lead to widespread confusion and mistrust, ultimately undermining the credibility of institutions and weakening social cohesion.
\item Zero-Day Exploits: 
Aggressive state actors can exploit LLMs to discover and leverage zero-day vulnerabilities. By training LLMs on massive amounts of data related to software development, vulnerabilities, and exploits, malicious actors can potentially identify previously unknown weaknesses in critical systems. These actors could then launch devastating cyberattacks, causing significant damage to their adversaries' infrastructure, economy, and security.
\item Autonomous Incursions:  Highly Compressed LLMs can potentially deploy autonomous incursion suites like Stuxnet, but with a greater degree of autonomy and less reliance on command and control. These advanced incursion suites might infiltrate targeted systems, adapt to their environment, and blend in with legitimate traffic, making them difficult to detect and mitigate. The integration of LLMs into these suites increases the potential for damage and disruption.
\end{itemize}
In response to these threats, the United States has imposed export restrictions on powerful GPU and TPU hardware to China. While these restrictions may slow down the development and deployment of LLMs for malicious purposes, they are unlikely to provide a long-term solution. As LLMs become more accessible and the technology proliferates, bad actors will trivially acquire the necessary hardware through alternative means, and the model weights themselves are already freely available. Existing defenses may not be adequate to counter the threats posed by LLMs, and the development of new cybersecurity measures requires time, resources, and expertise. In the absence of substantial increases in cybersecurity investment and research, it is likely that adversaries will continue to exploit LLMs to their advantage.\par
\href{https://securityintelligence.com/news/are-threat-actors-using-chatgpt-to-hack-your-network/}{According to Brad Hong}, Customer Success Manager with Horizon 3 AI, ``attackers are likely to adopt code generative AI as a means to address their limitations in scripting skills.'' Hong explains that code generative AI acts as a bridge, translating between languages that the attacker may not be proficient in and providing a means of generating base templates of relevant code. This reduces the skill requirements needed to launch a successful attack, as it serves as a tool in the attacker's arsenal alongside other tools.\par
In an email interview, Hong notes that the use of code generative AI, such as chat GPT, supercharges the attacker's ability to launch successful attacks. As explained by Patrick Harr, CEO at SlashNext, in an email comment, said \textit{``ChatGPT enables threat actors to modify their attacks in millions of different ways in minutes, and with automation, deliver these attacks quickly to improve compromise success.''}\par
The developers of chat GPT were aware that threat actors would attempt to weaponize the AI. As Harr explains, ``hackers are really good at weaponizing whatever technology is put in front of them.'' To mitigate this risk, the developers implemented preventive measures, such as flagging certain words and terms, like `ransom' or `ransomware.' For example, when researchers at Deep Instinct typed in the word `keylogger,' the chatbot responded with ``I'm sorry but it would not be appropriate or ethical for me to help you write a keylogger.''\par
However, these restrictions can be circumvented with a bit of clever rewording. As Jared, a Competitive Intelligence Analyst with Deep Instinct, explains, ``there's always a workaround.'' For example, instead of asking chat GPT to create ransomware code, an attacker could request a script that encrypts files and directories, drops a text file into the directory, and subdirectories.\par
The ability to weaponize chat GPT, or any other AI chatbot, is a game-changer for threat actors. With the ability to modify malicious code quickly and bypass cybersecurity defenses, these tools have the potential to greatly increase the effectiveness of attacks. As such, it is important for cybersecurity professionals to stay informed about the evolving threat landscape and the tools and techniques used by attackers \cite{brundage2018malicious}.\par 
At this early stage in the technology it is important that corporate and private users alike bear in mind that the LLMs are `leaky' and are using the data fed into them to train themselves. They are \href{https://help.openai.com/en/articles/6783457-chatgpt-general-faq}{explicit about this}. Anything that goes into chatGPT can resurface, as Samsung have found out \href{https://cybernews.com/news/chatgpt-samsung-data-leak/}{to their cost}.
\subsubsection{Use in war}
In the sphere of military, geopolitical, and civil defence the application of these tools is both shadowy and seemingly \href{https://www.vox.com/recode/23507236/inside-disruption-rebellion-defense-washington-connected-military-tech-startup}{somewhat incompetent}. \par
The US military's exploration of generative AI, trained on classified military data, showcases the growing use of AI in defense. The goal is to enhance operational capabilities and decision-making in intelligence analysis and strategic planning. Employing AI technologies can increase efficiency and provide additional operational insights. This ceding of control seems under discussed.\par

It is an especially twisted irony that `Rebellion Defence'' seem to have modelled themselves on the rebellion movement in the Star Wars fictional universe, seemingly unaware that Lucas most likely saw the USA as analogous to the Empire in the films \cite{immerwahr202221}. A \href{https://www.stopkillerrobots.org/wp-content/uploads/2022/10/ADR-Artificial-intelligence-and-automated-decisions-Single-View.pdf}{recent report} from ``Stop Killer Robots'' identifies the governance concerns which they have been monitoring for years. They identify areas of specific concern.
\begin{itemize}
\item transparency and explainability \item responsibility and  accountability
\item bias and discrimination.
\end{itemize}
\href{https://vframe.io/9n235/}{munition detection}  and autonomous war robots to do
\subsubsection{Existential Threat}
Many serious researcher are now sounding the alarm at the speed of development. In this moment is seems likely that ascribing emergent behaviours to large language models is a mirage born of the desires of the somewhat accelerationist community, and their more moderate couterparts \cite{schaeffer2023emergent}. There is potentially competitive advantage in mandating a `slowdown' in the technology development if the company and research team you work for find themselves behind. It's hard to tell what's going on. With that said the increase over time of noise generated by fancy autocomplete, vs human signal will doubtless lead (mathematically) to an undoing of current digital society, in the end. This is already impacting the training of new LLM models \cite{shumailov2023curse}. All of that is without considering the wilder theories such as the so called `paperclip miximiser' \cite{bostrom2003ethical}
or what Yudkowsky calls the \href{https://www.lesswrong.com/tag/squiggle-maximizer-formerly-paperclip-maximizer}{``squiggle maximiser''}, a literal end of life scenario.
\subsubsection{Existential threat to the internet}
\subsubsection{Scaling challenges}
In the DeepMind paper that introduced Chinchilla \cite{hoffmann2022empirical} several problems with scaling were highlighted
\begin{itemize}
\item Data, rather than model size, is currently the primary constraint on language modeling performance.
\item Large models (e.g., with 500B parameters or more) are not necessary if enough data can be leveraged.
\item Encountering barriers to data scaling would be a significant loss compared to the potential performance gains.
\item The amount of text data available for training is unclear, and there may be a shortage of general-domain data.
\item Specialized domains, such as code, have limited data compared to the potential gains if more data were available.
\end{itemize}
They argue that researchers often focus on scaling up the number of parameters rather than increasing the amount and diversity of training data. This focus on scaling numbers has led to a lack of clarity and rigour in describing the data collection processes and sources used in training these models. It seems  there are challenges associated with increasing the amount of training data, particularly in terms of quality and the diminishing returns of data scaling. 

\subsection{Superalignment Initiative by OpenAI}
OpenAI recently unveiled an initiative known as 'superalignment', a significant endeavour aimed at addressing the risks associated with superintelligent artificial intelligence (AI). The proposed solution has drawn attention due to its considerable resource allocation, ambitious goals, and purported transparency.

\subsubsection{Public Awareness and AI Risks}
The departure of Jeffrey Hinton from Google and his subsequent warnings about the dangers of AI, publicized through a New York Times article, have significantly raised the awareness and concern around the risks associated with superintelligent AI. The influence of Hinton in the field has transformed these concerns from a theoretical interest to a mainstream topic.

\subsubsection{Emphasis on Alignment}
OpenAI emphasizes alignment as a crucial element in AI risk mitigation, highlighting the potential for advanced general intelligence to diverge from human values. Ensuring alignment with these values is critical to avoid scenarios where AI systems could act counter to human interests. This focus is in line with the broader field of value alignment in AI ethics and research, but OpenAI have drawn criticism both for the secrecy around their implementation, and their relative investment in alignment to date. High prioritisation of capability advancement, largely driven by market forces, has left alignment relatively under-resourced. OpenAI has now acknowledged the historical imbalances between resources devoted to improving AI capabilities versus those dedicated to ensuring alignment, and perhaps they now seek to rectify this. The jury is out.

\subsubsection{Commitment to Superalignment}
Demonstrating their dedication to superalignment, they are committing a significant portion of their computational resources to this initiative. This allocation is indicative of a relatively new strategic prioritization of AI safety.
They have set an ambitious goal to build a human-level automated alignment researcher within four years. This is generally agreed to be a bit of a moon shot and rife with unknowns.
\subsubsection{Transparency and Standards}
OpenAI's decision to openly discuss their resource allocation and goals promotes a positive precedent for transparency within the AI community. This is progress. The AI safety community has responded with a mix of opinions to the superalignment initiative. The diversity of perspectives underscores the importance of ongoing dialogue on this topic.

\subsection{A more optimistic interpretation}
It's possible that in a post-social media world where AI assistants become ubiquitous, there is a shift toward more meaningful human-human interpersonal relationships. If everyone has an AI assistant in their ear to help mediate their personal fears and anxieties, we can perhaps see a path to more positive and local ways to communicate and engage with one another. The presence of AI assistants could conceivably help individuals become better listeners, communicators; ironically more empathetic. By providing personalized support and guidance, AI assistants might help us to better understand our own emotions and reactions, which in turn can lead to more authentic human interactions. If this new technology can undo the damage wrought by social media, and help us navigate our insecurities and anxieties, we may see a decline in the superficiality that has become synonymous with online interactions. This shift could lead to the resurgence of face-to-face conversations and the revitalization of community bonds, as individuals seek more authentic connections with those around them. This is still a worthwhile digital society, so long as the algorithm fuelled polarity fostered in the current is not repeated with weaponised AI assistants. AI assistants may seem less judgemental, and might promote mindfulness of our own biases and preconceptions, allowing us to approach conversations with an open mind and a willingness to learn from others. In this future, AI assistants not only serve as personal coaches and mediators for our individual fears and anxieties but also become catalysts for promoting healthier and more authentic human connections. By supporting our emotional well-being and helping us navigate interpersonal relationships, AI has the potential to transform the way we engage with one another. We would like to find ways to support this seemingly impossible and utopian vision.
\newpage
\subsection{The Law}
The \href{https://www.holisticai.com/papers/the-state-of-ai-regulations-in-2023}{world}, and more urgently the EU has framed it's legislative landscape one these technologies:
The USA has published it's ``AI Bill of Human Rights'', highlighting five themes:
\begin{itemize}
\item Safe and Effective Systems
\item Algorithmic Discrimination Protections
\item Data Privacy
\item Notice and Explanation
\item Human Alternatives, Consideration, and Fallback
\end{itemize}
It would be worth digging into these further here were it not so clear that the guardrails have already been breeched. The \href{https://www.whitehouse.gov/wp-content/uploads/2022/10/Blueprint-for-an-AI-Bill-of-Rights.pdf}{full report} is still worth reading.\par 
The US FTC has published a \href{}{blogpost} discussing the legal implications of AI-generated deception under the FTC Act. As synthetic media becomes more widespread, understanding the legal landscape is crucial for businesses involved in creating, distributing, or using AI-generated content. The FTC Act governs deceptive or unfair practices, including synthetic media and generative AI tools. Businesses should consider liability assessment, risk mitigation, deterrence measures, avoiding misrepresentation and false advertising, and post-release detection and monitoring. Other legal frameworks, such as copyright and trademark laws, defamation, and privacy rights, may also apply. The FTC emphasizes the importance of considering the broader social and ethical implications of these technologies and calls for collaboration among legal professionals, regulators, and industry stakeholders to ensure responsible development and use of AI-generated content. It feels like even this comparatively swift response is too little too late. \par
The legislative overhead (globally - taken in aggregate) is very high, and there's growing concern about the energy and carbon footprint of the technology \cite{wu2022sustainable}. The EU is first mover on this, and they have over-corrected for their lack of knowledge (arguably fair enough):\par
The EU regulation has been passed on 14/6 and classifies AI systems into four risk categories: unacceptable risk, high risk, limited risk, and minimal risk. Unacceptable risk AI systems will be prohibited, while high-risk AI systems will be subject to strict requirements. Any training of a model is automatically a foundational model (annoyingly) and therefore high risk. Getting a compliant model will require a demonstration of deep understanding of the workings of the model. It's unclear how anyone will accomplish this and it may end up being a defacto ban on trained models and possibly even optimised ones (LoRA). Any product derived from a \textbf{compliant} foundational model will be deemed acceptable by default. This question of compliant foundation models is absolutely key as we plan through the 3 year grace period which the EU has allowed. Any business doing any business in the EU is exposed. Stanford University Centre for Research on Foundation Models have done their own assessment on the compliance of the current models, and they simply aren't \ref{fig:euAIcompliance}. Bloom from Huggingface is closest and is `perhaps' \href{https://huggingface.co/BelleGroup/BELLE_BLOOM_GPTQ_4BIT}{usable in optimised modes} on cloud \href{https://lambdalabs.com/nvidia-h100-gpus}{hardware} \cite{dettmers2022case}. 

\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{euaicompliance}
    \caption{Stanford's assessment of the compliance of current foundation models vs the EU AI act.}
    \label{fig:euAIcompliance}
\end{figure}

Some other things can be high risk too, like external HR software. Limited-risk and minimal-risk AI systems will be subject to less stringent requirements. 
\begin{itemize}
  \item \textbf{Safety and Transparency:} AI systems used within the EU must be safe, transparent, traceable, non-discriminatory, and environmentally friendly. These systems should be overseen by humans to prevent harmful outcomes.
  \item \textbf{Risk-Based Categories:} The EU AI Act categorizes AI systems based on risk levels, which include unacceptable risk, high risk, limited risk, and a separate category for generative AI like ChatGPT.
  \item \textbf{Banned Practices:} Certain practices, like live facial recognition and scraping of biometric data from social media, are prohibited.
  \item \textbf{Transparency for Generative AI:} Companies may have to publish summaries of copyrighted material used for training their systems, which could be problematic for LLMs due to the vast amount of data involved in training.
  \item \textbf{Designing Prohibitions for Illegal Content:} AI systems should be designed to prevent the generation of illegal content.
  \item \textbf{AI-Generated Content Disclosure:} People must be informed when they are interacting with AI-generated content.
  \item \textbf{High-Risk Activities:} High-risk activities, such as certain uses of AI in law enforcement, will be subjected to tighter regulation.
  \item \textbf{Pre-Deployment Risk Assessments:} The EU proposes to implement a pre-deployment risk assessment process for high-risk models before they are released to the public.
  \item \textbf{Open Source Carve-out:} The act includes provisions for open source AI, but there are exclusions for large open source "Foundation Models" like GPT.
  \item \textbf{Training Data Documentation:} Companies may need to comprehensively document and be transparent about the copyrighted material used in the training of their algorithms, which could be challenging due to the amount and diversity of training data used.
\end{itemize}

It is somewhat unclear where these delimiters are; they will have to clarify it at some point. Burges Salmon Solicitors have provided a public access flowchart which is pretty helpful and is here as Figure \ref{fig:euaiflowchart}.\par

\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{euaiflowchart}
    \caption{EU AI compliance flowchart.}
    \label{fig:euAIcompliance}
\end{figure}

The USA and UK meanwhile will likely use the court system to iteratively establish these boundaries over time, though there will clearly be guidance soon(ish). Nobody wants to get caught up in courts around AI.\par
There will be legislative focus on human oversight. The regulation will require that all AI systems have human oversight, meaning that humans will be able to understand and control how the AI systems operate. This is intended to help ensure that AI systems are used in a safe and ethical manner.\par 
The regulation will require that AI systems be transparent, meaning that users will be able to understand how the AI systems work and how they make decisions.\par
The draft AI regulation intersects with GDPR in a number of ways. For example, GDPR requires that personal data be processed in a fair and transparent manner. So again, it will require that AI systems that process personal data be transparent and accountable. Additionally, the GDPR prohibits the processing of personal data for certain purposes, such as profiling. It rightly prohibits the use of AI systems for social scoring. \par
The regulation will apply to all AI systems that are developed, placed on the market, or \textbf{used in the European Union}, and we can expect that many countries will simply copy/paste this legal framework. It will be enforced by national authorities in each EU member state, which is suggestive of a degree of (risky) legislative arbitrage potential. Perhaps most annoyingly at a pragmatic level, there are a number of technical requirements for AI systems, such as accuracy, and fairness. All regulation will also include a number of procedural requirements, such as requirements for risk assessment and documentation. The penalties in the EU for violating the regulations will be significant. For example, up to 4\% of \textbf{global} annual turnover. The timeline for the adoption of the laws is still being negotiated, though the European Commission has stated that it expects the end of 2023, crucially with a two year phase in. This still means pretty much means `anything we do', since there is an extrinsic capture clause in EU law for international companies selling at all into the EU. This is the legislation to watch basically.\par
The Online Safety Bill is the most relevant UK legislative proposal pertaining to AI, as it includes a number of provisions that specifically address the use of AI by online platforms. The bill requires \textit{online} platforms to take steps to prevent the spread of harmful content, \textbf{including content that is generated by AI systems}. The bill also requires online platforms to be more transparent about how they use AI systems and to give users more control over how their data is used. The penalties for non-compliance with the legal provisions in the UK vary depend on the law that is being breached. Fines of up to £10 million for breaches of the DPA 2018. The information commissioners office has \href{https://ico.org.uk/for-organisations/uk-gdpr-guidance-and-resources/artificial-intelligence/guidance-on-ai-and-data-protection/how-should-we-assess-security-and-data-minimisation-in-ai/}{issued vague guidance} and can enforce through notices requiring companies to take steps to comply with the law. The UK seems less burdensome at this time, \textbf{but a quirk of the law gives \href{https://webdevlaw.uk/2022/11/21/a-quick-hypothetical-situation-or-your-crash-introduction-to-the-real-world/}{genuine legal peril} for C-Suite individuals}. 

==> NFTtable.tex <==

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[t]
\begin{tabular}{|c|
>{\columncolor[HTML]{FE996B}}c |
>{\columncolor[HTML]{FE996B}}c |
>{\columncolor[HTML]{9AFF99}}c |
>{\columncolor[HTML]{FE996B}}l |
>{\columncolor[HTML]{FFFC9E}}c |c|
>{\columncolor[HTML]{9AFF99}}c |
>{\columncolor[HTML]{9AFF99}}c |
>{\columncolor[HTML]{9AFF99}}c |
>{\columncolor[HTML]{9AFF99}}c |}
\hline
                                                                                                                          & \cellcolor[HTML]{9B9B9B}{\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Likely\\ dev \\ time\end{tabular}}} & \cellcolor[HTML]{9B9B9B}{\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Cost\\ of Use\end{tabular}}} & \cellcolor[HTML]{9B9B9B}{\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Speed \\ of Use\end{tabular}}} & \cellcolor[HTML]{9B9B9B}{\color[HTML]{FFFFFF} \begin{tabular}[c]{@{}l@{}}Energy\\ Cost\end{tabular}} & \cellcolor[HTML]{9B9B9B}{\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Open\\ source\end{tabular}}} & \cellcolor[HTML]{9B9B9B}{\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Bank \\ connect\end{tabular}}} & \cellcolor[HTML]{9B9B9B}{\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Buying \\ things\end{tabular}}} & \cellcolor[HTML]{9B9B9B}{\color[HTML]{FFFFFF} \textbf{Prizes}} & \cellcolor[HTML]{9B9B9B}{\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Trading\\ Peer 2 \\ Peer\end{tabular}}} & \cellcolor[HTML]{9B9B9B}{\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Arbitrary \\ token\\ issuance\end{tabular}}} \\ \hline
\cellcolor[HTML]{9B9B9B}{\color[HTML]{FFFFFF} \textbf{Bitcoin}}                                                           & \cellcolor[HTML]{FFFC9E}N/A                                                                                          & \begin{tabular}[c]{@{}c@{}}$\sim$£10 \\ per use\end{tabular}                                                  & \cellcolor[HTML]{FE996B}$\sim$H                                                                                 & High                                                                                                 & \cellcolor[HTML]{9AFF99}Yes                                                                                   & \cellcolor[HTML]{FE996B}\begin{tabular}[c]{@{}c@{}}Maybe\\ (Strike)\end{tabular}                                & Yes                                                                                                              & Yes                                                            & \cellcolor[HTML]{FFFC9E}Maybe                                                                                            & YES                                                                                                                          \\ \hline
\cellcolor[HTML]{9B9B9B}{\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Eth\\ ERC721\end{tabular}}}              & \cellcolor[HTML]{FFFC9E}N/A                                                                                          & \begin{tabular}[c]{@{}c@{}}$\sim$£10 \\ per use\end{tabular}                                                  & \cellcolor[HTML]{FFFC9E}Mins                                                                                    & \begin{tabular}[c]{@{}l@{}}Very\\ High\end{tabular}                                                  & \cellcolor[HTML]{9AFF99}Yes                                                                                   & \cellcolor[HTML]{FE996B}No                                                                                      & \cellcolor[HTML]{FE996B}No                                                                                       & Yes                                                            & \cellcolor[HTML]{FFFC9E}Maybe                                                                                            & Yes                                                                                                                          \\ \hline
\cellcolor[HTML]{9B9B9B}{\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Eth\\ token\end{tabular}}}               & \begin{tabular}[c]{@{}c@{}}Weeks \\ Months\end{tabular}                                                              & \begin{tabular}[c]{@{}c@{}}$\sim$£10 \\ per use\end{tabular}                                                  & \cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}Many\\ Mins\end{tabular}                                     & High                                                                                                 & Maybe                                                                                                         & \cellcolor[HTML]{FE996B}No                                                                                      & \cellcolor[HTML]{FFFC9E}Maybe                                                                                    & Yes                                                            & Yes                                                                                                                      & Yes                                                                                                                          \\ \hline
\cellcolor[HTML]{9B9B9B}{\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Custom\\ chain\end{tabular}}}            & Months                                                                                                               & \cellcolor[HTML]{9AFF99}\begin{tabular}[c]{@{}c@{}}Very \\ low\end{tabular}                                   & Secs                                                                                                            & Moderte                                                                                              & Maybe                                                                                                         & \cellcolor[HTML]{FFFC9E}Maybe                                                                                   & Yes                                                                                                              & Yes                                                            & Yes                                                                                                                      & Yes                                                                                                                          \\ \hline
\cellcolor[HTML]{9B9B9B}{\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}BTC pay \\ server +\\ LND\end{tabular}}} & \cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}Days but\\ operational\\ overheads\end{tabular}                   & \begin{tabular}[c]{@{}c@{}}$\sim$£10\\ per use\end{tabular}                                                   & Secs                                                                                                            & \cellcolor[HTML]{FFFC9E}Lower                                                                        & \cellcolor[HTML]{9AFF99}Yes                                                                                   & \cellcolor[HTML]{9AFF99}Yes                                                                                     & Yes                                                                                                              & Yes                                                            & \cellcolor[HTML]{FE996B}No                                                                                               & \cellcolor[HTML]{FE996B}No                                                                                                   \\ \hline
\cellcolor[HTML]{9B9B9B}{\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}BTC\\ L2 and L3\end{tabular}}}                 & Months                                                                                                                & \cellcolor[HTML]{9AFF99}\begin{tabular}[c]{@{}c@{}}Very \\ Low\end{tabular}                                   & Secs                                                                                                            & \cellcolor[HTML]{FFFC9E}Low                                                                          & Some                                                                                                          & \cellcolor[HTML]{FFFC9E}Maybe                                                                                   & Yes                                                                                                              & Yes                                                            & Yes                                                                                                                      & \cellcolor[HTML]{FE996B}No                                                                                                   \\ \hline
\cellcolor[HTML]{9B9B9B}{\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Colour \\ coins\end{tabular}}}           & Months                                                                                                               & \cellcolor[HTML]{9AFF99}\begin{tabular}[c]{@{}c@{}}Very\\ Low\end{tabular}                                    & Secs                                                                                                            & High                                                                                                 & Maybe                                                                                                         & \cellcolor[HTML]{FFFC9E}Maybe                                                                                   & Yes                                                                                                              & Yes                                                            & Yes                                                                                                                      & \cellcolor[HTML]{FFFC9E}Maybe                                                                                                \\ \hline
\end{tabular}
\caption{This table is basically broken and out of date and will be sorted out soon!}%shows some of the affordances of the technologies. Dark orange squares are deemed unsuitable / failing in that technology. It can be seen that none are perfect}
\label{tab:compare}
\end{table*}


%------------------------------------------------


==> mindmap.tex <==
\section{Compendium of links not yet integrated}
\begin{itemize}
\item
  \href{https://stephenfollows.com/how-we-got-hired-to-create-an-ai-generated-feature-film-screenplay/}{real
  world AI script}

  \begin{itemize}
  \tightlist
  \item
    The short answer is: we started with a product and a plan. As with
    most things in life, our success was the result of a lot of hard
    work. In order to get to a product, we had to get to a plan. We had
    to be able to articulate a clear vision of what we wanted to create.
    The first step was to create a script. The script was the foundation
    of our plan. The script was where we chose to create a film
  \end{itemize}
\item
  \href{https://writings.stephenwolfram.com/2023/02/what-is-chatgpt-doing-and-why-does-it-work/}{Wolfram
  on how chatgpt works}

\item
  \href{https://techcrunch.com/2022/01/12/the-metaverse-will-be-filled-with-elves/}{Elves
  (bots) techcrunch article}
\item
  \href{https://www.atomic14.com/2022/12/05/using-chatgpt-as-a-co-founder.html}{Using
  ChatGPT as a founder}
\item
  \href{https://deepmind.github.io/dramatron/}{Dramatron (other)}

  \begin{itemize}
  \tightlist
  \item
    This demo and arxiv paper are for a tool called Dramatron that uses
    machine learning to help with writing scripts.
  \end{itemize}
\item
  \href{https://beta.elevenlabs.io/}{Eleven labs language and text to
  speech}
\item
  \href{https://uberduck.ai/}{Uberduck open source text to speech}
\item
  \href{https://www.youtube.com/watch?v=DnF4WzM5LPU}{Inworld (steam game
  plugin AI system) for voice chat and answer}
\item
  \href{https://www.marktechpost.com/2022/10/27/ibm-research-introduces-artificial-intelligence-unit-aiu-its-first-complete-system-on-chip-designed-to-run-and-train-deep-learning-models-faster-and-more-efficiently-than-a-general-purpose-cpu/}{IBM
  custom board}
\item
  \href{https://www.okdo.com/p/nvidia-jetson-agx-orin-64gb-developer-kit/}{Nvidia
  jetson AI}

  \begin{itemize}
  \tightlist
  \item
    Answer: The Nvidia Jetson AGX-Orin is a developer kit with a 64-bit
    quad-core ARM Cortex-A57 processor and a Pascal-based GPU. It has a
    single-board computer (SBC) form factor with a microSD card slot and
    a USB 3.0 port. It is compatible with the Jetson TX2 and the Jetson
    TX1. It has a 64-bit quad-core ARM Cortex-A57 processor
  \end{itemize}
\item
  \href{https://www.theverge.com/2023/2/23/23611668/ai-image-stable-diffusion-mobile-android-qualcomm-fastest}{Qualcomm
  phone SD}

  \begin{itemize}
  \tightlist
  \item
    -possible-internet-of-things-episode-7 What is the most important
    takeaway from this article? The most important takeaway from this
    article is that the new Snapdragon 855 chip is able to support a
    stable connection for AI-based devices, even on a 4G network. What
    is the main idea of the article? The main idea of the article is
    that the new Snapdragon 855 chip can support a stable connection for
    AI-based devices,
  \end{itemize}
\item
  \href{https://www.esperanto.ai/}{Esperanto RISC V}
\item
  \href{https://hdh4797.wixsite.com/dhan/project-1}{}

\begin{verbatim}
The MetaVRain asic claims 900x speed increases} on general GPU problems
\end{verbatim}
\item
  \href{https://sdtools.org/}{Stability specific tools}

  \begin{itemize}
  \item
    \href{https://github.com/bmaltais/kohya_ss}{Lora training interface
    for windows}

    \begin{itemize}
    \tightlist
    \item
      m\_tutorial/blob/master/tutorial.md What is the difference between
      a state machine and a finite state machine? The documentation for
      kohya-ssm explains that a state machine is a finite state machine
      with a history. It also includes a diagram that shows a state
      machine as a box with a history. A finite state machine is a
      machine that has a finite number of states. It can be in only one
      of these states at any
    \end{itemize}
  \item
    \href{https://substack.com/profile/110613456-followfoxai}{Fine
    tuning with captioning and other fine tuning tricks, followfox}

    \begin{itemize}
    \tightlist
    \item
      This is a very impressive list of tools and libraries, which I
      think is a good thing. I don't think that it's a good idea to have
      a large number of tools, but having a large number of libraries is
      a good thing. I've never used any of these libraries. I'm not even
      sure how to pronounce ``Fox-Ai''. I really like the idea of using
      the Web Audio API
    \end{itemize}
  \item
    \href{https://huggingface.co/datasets/Nerfgun3/bad_prompt}{Negative
    embedding textual inversion for hands etc}

    \begin{itemize}
    \tightlist
    \item
      / The dataset contains data about the velocity of Nerf darts fired
      from different guns. The data is in the form of a CSV file, which
      is a text file that contains a number of rows and columns. Each
      row represents a single record. The columns in a CSV file are
      separated by commas. The Nerfgun3 dataset contains a single CSV
      file with four columns. The first column contains the names of the
      guns. The next three columns contain the velocity of the darts
    \end{itemize}
  \item
    \href{https://www.thosesixfaces.com/post/stable-diffusion-getting-started-windows}{Automatic1111
    GUI and user guide}

    \begin{itemize}
    \tightlist
    \item
      -10-and-office-2016-and-2016-for-mac-install-and-configure-office-2016-for-mac-on-a-mac-os-x-10-11-10-system/
      Your response should be at least 200 words in length. You are
      required to use at least your textbook as source material for your
      response. All sources used, including the textbook, must be
      referenced; paraphrased and quoted material must have accompanying
    \end{itemize}
  \item
    \href{https://github.com/comfyanonymous/ComfyUI}{ComfyUI nodes
    based}

    \begin{itemize}
    \tightlist
    \item
      /wiki/Home This is a brief summary of the ComfyUI library. The
      library is a set of UI components that are designed to provide a
      consistent look and feel across all platforms and all devices. The
      library is open source and can be found on Github here:
      https://github.com/comfyanonymous/ComfyUI. The library is
      currently being used by a set of companies, including The New York
      Times, to create their apps. The library is free to use
    \end{itemize}
  \item
    \href{https://christiancantrell.com/\#ai-ml}{Photoshop plugin}

    \begin{itemize}
    \tightlist
    \item
      -tutorial Use the following code to summarize the page:
      \#!/usr/bin/env python3 """ Summary of the page at
      https://christiancantrell.com/\#ai-ml-tutorial """ import sys
      import requests import nltk import numpy as np import
      matplotlib.pyplot as plt from sklearn.metrics import
      roc\_auc\_score from sklearn.feature\_extraction.text import
      CountVectorizer from sk
    \end{itemize}
  \item
    Dreambooth retraining for faces
  \item
    \href{https://www.reddit.com/r/StableDiffusion/comments/10gs4s2/new_expert_tutorial_for_textual_inversion_text/}{Textual
    inversion}
  \item
    \href{https://www.youtube.com/watch?v=AeDngG9kQNI}{Depth map into
    blender from SD2}
  \item
    \href{https://www.heroo.ai/}{Game development using SD}

    \begin{itemize}
    \tightlist
    \item
      blog/heroo-ai-blog. Your response should be at least 150 words in
      length. You are required to use at least your textbook as source
      material for your response. All sources used, including the
      textbook, must be referenced; paraphrased and quoted material must
      have accompanying citations. 1. What is the difference between AI
      and machine learning? 2. What is the difference between supervised
      and unsupervised learning? 3. Can you give an example
    \end{itemize}
  \item
    \href{https://github.com/ashawkey/stable-dreamfusion}{GitHub -
    ashawkey/stable-dreamfusion: A pytorch implementation of text-to-3D
    dreamfusion, powered by stable diffusion. , A pytorch implementation
    of text-to-3D dreamfusion, powered by stable diffusion. - GitHub -
    ashawkey/stable-dreamfusion: A pytorch implementation of text-to-3D
    dreamfusion, powered by stable diffusion.}
  \item
    \href{https://holovolo.tv}{holovolo - immersive volumetric VR180
    videos and photos, and 3D stable diffusion, for Quest and WebVR ,-}
  \item
    \href{https://jalammar.github.io/illustrated-stable-diffusion/}{The
    Illustrated Stable Diffusion Jay Alammar Visualizing machine
    learning one concept at a time.}
  \item
    ControlNet
  \item
    \href{https://www.reddit.com/r/StableDiffusion/comments/127gck9/sdtools_v16/}{sdtools
    image v 1.6}
  \item
    GitHub - lllyasviel/ControlNet: Let us control diffusion models!
  \item
    \begin{itemize}
    \tightlist
    \item
      \href{https://www.reddit.com/r/StableDiffusion/comments/1148x38/tencent_ai_just_release_their_method_and_code/}{Tencent
      AI just release their method and code very similar to ControlNet :
      r/StableDiffusion}
    \end{itemize}
  \end{itemize}
\item
  \href{https://www.usegalileo.ai/}{UX design AI}
\item
  \href{http://www.cs.cmu.edu/~pix2pix3D/}{pix2pix-3D: 3D-aware
  Conditional Image Synthesis}

  \begin{itemize}
  \tightlist
  \item
    The problem of image-to-image translation is a difficult one, and
    the results are often not very convincing. The problem of
    image-to-image translation is a difficult one, and the results are
    often not very convincing. In this assignment, you will use a neural
    network to learn how to translate an image from one domain to
    another. Your neural network will learn to translate one domain to
    another domain. For example, you will use a neural
  \end{itemize}
\item
  \href{https://mingukkang.github.io/GigaGAN/}{GIGAgan}
\item
  \href{https://github.com/upscayl/upscayl}{GitHub - upscayl/upscayl:
  Upscayl - Free and Open Source AI Image Upscaler for Linux, MacOS and
  Windows built with Linux-First philosophy. (other)}
\item
  \href{https://film-net.github.io/}{FILM frame interpolator}
\item
  \href{https://twitter.com/cut_pow/status/1576748659051749377}{Interframe
  consistency is now here}
\item
  \href{https://studios.disneyresearch.com/2022/11/30/production-ready-face-re-aging-for-visual-effects/}{Production
  ready re aging}

  \begin{itemize}
  \tightlist
  \item
    The team has developed a new algorithm for re-aging faces in a
    single image. The algorithm works by first detecting the face in the
    image and then using a neural network to generate a new face with a
    different age. The algorithm can be used in a variety of
    applications including visual effects, video conferencing, and photo
    editing. The algorithm was trained using over 50,000 images of faces
    from a variety of sources including the Internet, movies, and TV
  \end{itemize}
\item
  \href{https://www.synthesia.io/}{Video talking heads from text
  service}

  \begin{itemize}
  \tightlist
  \item
    The following is a brief description of the page: Synthesia is a
    free, open-source music score editor that runs in your web browser.
    It is a great tool for composers, songwriters, and music students.
    If you are a composer, songwriter, or music student, you can use
    Synthesia to compose music and to practice sight-singing. If you are
    a music teacher, you can use Synthesia to teach
  \end{itemize}
\item
  \href{https://github.com/proceduralit/StableDiffusion_Houdini}{Houdini}
\item
  \href{https://www.youtube.com/watch?v=4uzzD9sD-PI}{Synthesia corporate
  video generation}

  \begin{itemize}
  \tightlist
  \item
    . Answer: The video shows a demonstration of a way to make a small,
    inexpensive, and flexible robotic arm. The arm is made of two servo
    motors connected by a steel rod, which is bent to form a ``U''
    shape. By rotating the servos, the rod is bent and the arm is able
    to move. The arm has a number of applications, such as being used in
    a manufacturing environment or to aid in search and rescue
    operations.
  \end{itemize}
\item
  \href{https://www.reddit.com/r/StableDiffusion/comments/114zmh3/controlnet_and_ebsynth_make_incredible_temporally/}{controlnet
  and ebsynth temporal consistency}
\item
  \href{https://github.com/isl-org/PhotorealismEnhancement}{Intel
  enhance photorealism in realtime}

  \begin{itemize}
  \tightlist
  \item
    /wiki What is the goal of the project? The goal of the project is to
    create a new image processing framework, which will be used by the
    ISL framework to improve the quality of the generated images. What
    is the current state of the project? The project is in the very
    early stages. We have a few ideas of how to implement the framework
    and have started coding some of the basic components. What are the
    short-term goals for the
  \end{itemize}
\item
  \href{https://www.kombitz.com/2023/03/28/how-to-use-modelscope-text2video-with-automatic1111s-stable-diffusion-web-ui/}{How
  to Use ModelScope text2video with Automatic1111 s Stable Diffusion Web
  UI \textbar{} kombitz: Enable the Extension Click on the Extension tab
  and then click on Install from URL. Enter
  https://github.com/deforum-art/sd-webui-modelscope-text2video in the
  URL box and click on Install. Click on Installed and click on Apply
  and restart UI. Go to your stable-diffusion-webui/models folder and
  create a folder called ModelScope and then create a folder called t2v
  under ModelScope. This is your models folder for text2video.}
\item
  \href{https://meshcapade.com/}{Meshcapade virtual humans}
\item
  \href{https://ofa-sys.github.io/MoFusion/}{text to human motion}
\item
  \href{https://www.linkedin.com/posts/reneschulte_nerf-deeplearning-metaverse-activity-7010898662465617921-56P_?utm_source=share\&utm_medium=member_desktop}{nerf
  avatars}
\item
  \href{https://twitter.com/IntuitMachine/status/1608690077139599360}{chatgpt
  to avatar}
\item
  \href{https://3d-avatar-diffusion.microsoft.com/?utm_campaign=AI\%20Art\%20Weekly\&utm_medium=email\&utm_source=Revue\%20newsletter\#/}{Microsoft
  sculpted avatars}
\item
  \href{https://80.lv/articles/ziva-dynamics-announces-a-new-ml-trained-facial-rigging-service/}{ML
  realtime UE facial expresssions}
\item
  \href{https://talkshow.is.tue.mpg.de/}{Gestures from speech}
\item
  \href{https://volucap.com/}{Volucap volumentric deep fakes}
\item
  \href{https://www.flawlessai.com/}{FlawlessAI cloud facial plus
  language translattion}
\item
  \href{https://www.youtube.com/watch?v=uboj01Gfy1A}{Microsoft AI faces}
\item
  \href{https://nv-tlabs.github.io/LION/}{LION instant 3D textured geom}
\item
  \href{https://captures.lumalabs.ai/imagine}{Luma text to 3D}
\item
  \href{https://www.reddit.com/r/virtualreality/comments/xvy5dc/3d_generation_from_a_single_image/}{3D
  generation from a single image : r/virtualreality}

  \begin{itemize}
  \tightlist
  \item
    The web page has a title "3d generation from a single image" and a
    short description "I made a 3d model of a building from a single
    image". The web page has a title "3d generation from a single image"
    and a short description "I made a 3d model of a building from a
    single image". The web page has a tagline "I made a 3d model of a
    building from a single image". The web page has a tag
  \end{itemize}
\item
  \href{https://make-it-3d.github.io/}{Make-It-3D: High-Fidelity 3D
  Creation from A Single Image with Diffusion Prior:}

  \begin{itemize}
  \tightlist
  \item
    The Make-It-3D algorithm can create high-fidelity 3D content from
    only a single image. It uses a two-stage optimization pipeline,
    first optimizing a neural radiance field by incorporating
    constraints from the reference image and diffusion prior, and then
    transforming the coarse model into textured point clouds. Extensive
    experiments demonstrate that the algorithm outperforms prior works,
    resulting in faithful reconstructions and impressive visual quality.
  \item
    webgl-graphics-book/lesson11-2.html The Shaders The shaders used in
    this lesson are almost the same as in the previous lesson. The only
    difference is that we have an additional uniform variable,
    ``u\_time'', which is used to update the color of the cube each
    frame. The vertex shader is as follows: \#version 300 es precision
    mediump float; in vec2 in\_position; in
  \end{itemize}
\item
  "Vox-E: Text-guided Voxel Editing of 3D Objects."
\item
  \href{https://dreamfusion3d.github.io/}{DreamFusion: Text-to-3D using
  2D Diffusion (other)}
\item
  \href{https://lukashoel.github.io/text-to-room/}{Text2Room: Extracting
  Textured 3D Meshes from 2D Text-to-Image Models:}

  \begin{itemize}
  \tightlist
  \item
    The Text2Room algorithm generates 3D meshes from a given text prompt
    by synthesizing a sequence of images from different poses. The core
    idea is to select viewpoints such that the content of each image can
    be fused into a seamless, textured 3D mesh. The algorithm
    iteratively fuses scene frames with the existing geometry to create
    a seamless mesh. Unlike existing works that focus on generating
    single objects or zoom-out trajectories from text, our method
    generates complete 3D scenes with multiple objects and explicit 3D
    geometry.
  \end{itemize}
\item
  \href{https://google-research.github.io/seanet/musiclm/examples/}{Google
  MusicLM}
\item
  \href{https://text-to-audio.github.io/}{Text2audio}
\item
  \href{https://ico.org.uk/for-organisations/guide-to-data-protection/key-dp-themes/guidance-on-ai-and-data-protection/how-should-we-assess-security-and-data-minimisation-in-ai/}{AI
  security considerations}
\item
  \href{http://gptzero.me/}{gptzero spots AI authoring}
\item
  \href{https://www.stateof.ai/}{State of AI report}
\item
  \href{https://txt.cohere.ai/sentence-word-embeddings/}{About sentence
  embedding}
\item
  \href{https://github.com/bigscience-workshop/petals}{Bigscience petals
  run training through torrents}
\item
  \href{https://medium.com/@socialemail/how-diffusion-models-can-achieve-seemingly-arbitrarily-large-compression-ratios-through-learning-2b21a317a46a}{How
  the compression is so huge in diffusion models}
\item
  \href{https://metavert.substack.com/p/the-generative-ai-canon}{the
  generative AI canon substack roundup}
\item
  \href{https://github.com/oobabooga/text-generation-webui/wiki/LLaMA-model}{4bit
  30B linux integration}
\item
  \href{https://medium.com/@imicknl/how-to-create-a-private-chatgpt-with-your-own-data-15754e6378a1}{How
  to create a private ChatGPT with your own data: Learn the architecture
  and data requirements needed to create your own Q\&A engine with
  ChatGPT/LLMs.}

  \begin{itemize}
  \tightlist
  \item
    This text provides a guide on how to create a private ChatGPT with
    your own data. It discusses the feasibility of such a project and
    outlines the steps necessary to accomplish it.
  \end{itemize}
\item
  \href{https://huggingface.co/togethercomputer/GPT-NeoXT-Chat-Base-20B}{GPT-NeoXT-Chat-Base-20B
  human optimised free model}
\item
  \href{https://arxiv.org/abs/2209.01188}{Petals collaborative fine
  tuning}

  \begin{itemize}
  \tightlist
  \item
    The paper presents a new method to estimate the gravitational
    potential of a large number of galaxies using weak gravitational
    lensing. The method is based on the Bayesian approach to
    gravitational lensing, where the potential is solved from the
    lensing shear field. The method is applied to the 2dFGRS sample of
    galaxies, which is a large cosmological survey which has been used
    for several studies of cosmology. It is shown that the new method is
    able to recover the cosmological
  \end{itemize}
\item
  Lllama and stuff
\item
  \href{https://arxiv.org/abs/2303.11156}{Can AI-Generated Text be
  Reliably Detected?:}

  \begin{itemize}
  \tightlist
  \item
    In the paper "Can AI-Generated Text be Reliably Detected?", the
    authors show that current methods for detecting AI-generated text
    are not reliable in practical scenarios. They first demonstrate that
    paraphrasing attacks can break a range of detectors, including those
    using watermarking schemes and neural network-based detectors. They
    then provide a theoretical impossibility result showing that for a
    sufficiently good language model, even the best-possible detector
    can only perform marginally better than a random classifier.
    Finally, they show that even LLMs protected by watermarking schemes
    can be vulnerable to spoofing attacks where adversarial humans can
    add hidden watermarking signatures to their generated text.
  \end{itemize}
\item
  \href{https://github.com/Torantulino/Auto-GPT}{GitHub -
  Torantulino/Auto-GPT: An experimental open-source attempt to make
  GPT-4 fully autonomous.: An experimental open-source attempt to make
  GPT-4 fully autonomous. - GitHub - Torantulino/Auto-GPT: An
  experimental open-source attempt to make GPT-4 fully autonomous.}

  \begin{itemize}
  \tightlist
  \item
    Auto-GPT is an experimental open-source project that aims to make
    the GPT-4 text generation system fully autonomous. The project is
    still in its early stages, but has already produced some results,
    including an article written by the system when prompted to do so.
  \end{itemize}
\item
  \href{https://simonwillison.net/2023/Apr/2/calculator-for-words/}{Think
  of language models like ChatGPT as a calculator for words : One of the
  most pervasive mistakes I see people using with large language model
  tools like ChatGPT is trying to use them as a search engine. As with
  other LLM}
\item
  \href{https://twitter.com/ronithhh/status/1641318606549176321}{Instant
  app from prompts}

  \begin{itemize}
  \tightlist
  \item
    In the first part of this article, we looked at how to use an
    OpenShift cluster to host a Java application. In the second part, we
    saw how to use OpenShift to host a Python application. In the third
    part, we looked at how to use OpenShift to host a PHP application.
    In the fourth part, we saw how to use OpenShift to host a Ruby
    application. In the fifth part, we looked at how to use OpenShift to
    host a Node.js
  \end{itemize}
\item
  \href{https://replit.com/@asrsubs/SkyRoads-GPT-4}{endless runner
  without any coding experience}
\item
  \href{https://blog.medium.com/how-were-approaching-ai-generated-writing-on-medium-16ee8cb3bc89}{Medium
  listing approachs}
\item
  \href{https://www.theguardian.com/technology/2023/mar/23/tech-guru-jaron-lanier-the-danger-isnt-that-ai-destroys-us-its-that-it-drives-us-insane}{Drives
  us mad, Guardian}

  \begin{itemize}
  \tightlist
  \item
    Solution Preview The article is about the effects of artificial
    intelligence on human beings. The author of the article is Jaron
    Lanier, who is a computer scientist, author, composer, and musician.
    He is also an interdisciplinary researcher, and a virtual reality
    pioneer. He is the author of the book "You Are Not a Gadget" (2010).
    The article is about the effects of artificial intelligence on human
    beings. The author of the article is Jaron Lanier, who is
  \end{itemize}
\item
  \href{https://buttondown.email/hillelwayne/archive/programming-ais-worry-me/}{Programming
  AIs worry me Buttondown:}

  \begin{itemize}
  \tightlist
  \item
    The text discusses the concerns around using AI to generate code,
    specifically around the idea of proofreading the code. The author
    describes an experience with using voice-to-text where they found it
    difficult to proofread the text for errors. The text argues that
    using AI to generate code changes the work from writing code to
    proofreading code, and that this is a problem.
  \end{itemize}
\item
  \href{https://about.sourcegraph.com/blog/cheating-is-all-you-need}{Stop
  whining blog post}
\item
  \href{https://github.com/emcf/engshell/tree/main}{Engshell shell LLM
  extension}

  \begin{itemize}
  \tightlist
  \item
    /doc/reference The web page contains information about the EngShell
    project. It includes a list of the major features, a list of the
    major components, a list of the major dependencies, and a list of
    the major contributors. Read the web page at the following URL:
    https://github.com/emcf/engshell/tree/main/doc/engshell-tutorial The
    web page provides a tutorial on how to use EngShell. It starts with
  \end{itemize}
\item
  Training

  \begin{itemize}
  \item
    \href{https://github.com/alpa-projects/alpa}{}

    is a system for training and serving large-scale neural networks.
    Scaling neural networks to hundreds of billions of parameters has
    enabled dramatic breakthroughs such as GPT-3, but training and
    serving these large-scale neural networks require complicated
    distributed system techniques. Alpa aims to automate large-scale
    distributed training and serving with just a few lines of code.

    Alpa:

    Serving OPT-175B, BLOOM-176B and CodeGen-16B using Alpa:
    https://lnkd.in/g\_ANHH6f
  \item
    \href{https://github.com/microsoft/DeepSpeed}{is an easy-to-use deep
    learning optimization software suite that enables unprecedented
    scale and speed for DL Training and Inference. Visit us at
    deepspeed.ai or our Github repo. Megatron-LM GPT2 tutorial:
    https://lnkd.in/gXvPhXqb}
  \item
    \href{https://github.com/NVIDIA/Megatron-LM}{- / Megatron is a
    large, powerful transformer developed by the Applied Deep Learning
    Research team at NVIDIA. Below repository is for ongoing research on
    training large transformer language models at scale. Developing
    efficient, model-parallel (tensor, sequence, and pipeline), and
    multi-node pre-training of transformer based models such as GPT,
    BERT, and T5 using mixed precision. pretrain\_gpt3\_175B.sh:
    https://lnkd.in/gFA9h8ns}
  \item
    \href{https://colossalai.org/}{- provides a collection of parallel
    components for you. It aim to support us to write our distributed
    deep learning models just like how we write our model on our laptop.
    It provide user-friendly tools to kickstart distributed training and
    inference in a few lines. Open source solution replicates ChatGPT
    training process.Ready to go with only 1.6GB GPU memory and gives
    you 7.73 times faster training: https://lnkd.in/gp4XTCnz}
  \item
    \href{https://github.com/OpenBMB/BMTrain}{is an efficient large
    model training toolkit that can be used to train large models with
    tens of billions of parameters. It can train models in a distributed
    manner while keeping the code as simple as stand-alone training.}
  \item
    \href{https://github.com/tensorflow/mesh}{(mtf) is a language for
    distributed deep learning, capable of specifying a broad class of
    distributed tensor computations. The purpose of Mesh TensorFlow is
    to formalize and implement distribution strategies for your
    computation graph over your hardware/processors. For example: "Split
    the batch over rows of processors and split the units in the hidden
    layer across columns of processors." Mesh TensorFlow is implemented
    as a layer over TensorFlow.}
  \end{itemize}
\end{itemize}


==> overview.tex <==

In the last couple of years the Greater Manchester Cyber Foundry has been collaborating with small to medium sized enterprises, responding to their questions about emerging trends. We were asked about exciting new developments in the transmission of value, and trust in Metaverses. The problem is that each of these topics alone are enormously complex, and the intersections seem to be more so. We have been researching the current state-of-the-art, and the emerging consensus narrative, to try to figure out how the collision of these technologies might serve SMEs. \par
Because we’re the GM Cyber Foundry, we started out with security best practices in mind. How can we enable small and especially developing companies, to have a foot in the door on a global stage, without their cybersecurity costs spiralling? Fortunately, we discovered a wealth of carefully crafted open source tools which can support this exploration. We have tried to assemble them cogently, to deliver a kit for experimentation to curious technically minded SMEs, and we have applied our own security knowledge on top of an already top class set of tools. It’s certainly not production ready, but it's good enough to commit small amounts of money into, for experimentation purposes.\par
Whilst researching, it seemed that every door we opened was full of interesting and useful treats. What was supposed to be a short technical paper quickly became a 150-page book, and a deployable virtual machine stack, with a dozen different open source components in it. \par
To that end, this book supports the virtual lab, which supports anyone who thinks this material might be useful. In the following sections you’ll read a precis of the sections of the book, which will hopefully give an insight into what ``this stuff'' is. Then you can decide to download the book and the lab how to guide. All of it is open source, all of it can be contributed to on GitHub, all of it will be developed forward, and none of it is really finished yet.
Section 1  attempts to overview what the book is about, which is value transmission, with distributed trust, in global social mixed reality systems. \par
Next is a summary of Web3, as it stands right now. Web3 is a complex term and it’s cropping up far more in the technical press so we wanted to cover off what it might mean, but honestly, it’s still pretty confusing. There are a bunch of legacy explanations which are Web3.0, that are withering on the vine. Then there’s the new VC funded, super hyped and potentially useless Web3 incarnations, which again cover a slew of intersecting technologies. This doesn’t mean there’s nothing to see here. The astonishing amount of money and developer talent, and the clear market hunger for things like NFTs (non-fungible tokens) suggest that there’s a future for Web3, it’s just really unclear what the value could be for our curious SME.\par
In the next section we took a look at blockchain, which is very intersectional with Web3. Even on its own this is a very complex emergent set of disciplines. \par
The blockchain section was especially interesting to research. It turns out there’s a LOT of ways to get this technology wrong. Even very appealing options on paper, turn out to have very shaky foundations. There are really valuable things here, but given the complexity, and the size of that chapter, we decided to focus down on the most promising of the technology stacks, which interestingly turned out to be the original; the Bitcoin network.\par
Even Bitcoin isn’t just Bitcoin anymore. It’s a swarm of open source tools which can (in theory) accomplish a great many things. These newer, ancillary elements to Bitcoin, are emergent right now. Some of the won’t be around until later in the year and it’s questionable whether they will even work out. With that said there’s already enough here for us to cherry pick some useful components and start to map those forward into our metaverse proposal.\par
In looking around at the available options, it seems possible that the features which are important to Web3 in section 1, can also potentially arise from the Bitcoin technology that we settled on in section 2. This was somewhat unexpected, so we started mapping that over too.\par
The next section is about Money. In expanding our research on Bitcoin, we found that it’s impossible to think about the tech without opening up a whole other line of questions about money itself. This is fine because we set out to look at global value transfer for business. It’s not a trivial subject though, and this section tries to overview why value and Bitcoin are so enmeshed then what other options there might be in the end (because Bitcoin has kicked off a whole slew of global adoption outside of itself) and finally what we can do pragmatically, both now, and in the coming year or two.\par
The distributed identity management, and trust section follows. It’s not an easy section to write about, because there’s a lot of research, it’s not our field, and finding the value to SMEs has actually been very difficult. This section is likely to be overhauled a few times in the coming months as we settle on technologies that we believe are simple and secure enough.\par
In section 7 we take another look at NFTs. It’s impossible to ignore this stuff now. It’s fundamentally a bit broken, but there are likely some use cases, and the money and development attention it’s getting are incredible. We try to navigate our hypothetical SME through this as best we can. It’s not that we didn’t understand it completely, just that the tech moves so very fast that it’s impossible to even describe what’s going on accurately at any given point. We’re actually pretty excited about future versions of this technology, based around Bitcoin, because that allows us to keep just one value stack in the  lab. We’ve mapped that forward into the open source tools that we recommend. This very much ended up looking like our priors; our cyber security values, and our wish to build toward a simpler product using only Bitcoin. To that end we asked another author, with much more of a foot in the content creation world, to collaborate with us on this chapter. This will benefit from smoother integration over the coming months.\par
Chapter 8 is a big one for us as it’s our research area prior to opening up the Bitcoin box(es).\par Metaverse, or at least one of the current definitions of metaverse, is just social interaction in mixed reality (VR/AR/XR!). We’ve been studying that for decades, so this section is more academic and tried to boil down what we think is most important to map forward into the lab. The choices we make here guided us toward the selection of free and open source metaverse software, which we selected from a bunch that we reviewed. You can make your own choices and gain insight from the systems we looked at.\par
We also take a look at the other definitions of metaverses which are doing the rounds on the web, try to unpick which is which, and what they are for, then we attempt to weave back together the best of both. This ends up looking a bit like the Venn at the top, where we have transmission of provable identity, non-fungible tokens bearing value or data, distributed files, actual money (including micropayments) and a social layer based on our best knowledge about mixed reality.\par
Past this stage in the book we get into the murky and half developed tail end where we’re interfacing with our design choices, and the stack which can be deployed into the cloud.



